Probabilistic Stability Guarantees for Feature Attributions

Stability guarantees have emerged as a principled way to evaluate feature attributions, but existing certification methods rely on heavily smoothed classifiers and often produce conservative guarantees. To address these limitations, we introduce soft stability and propose a simple, model-agnostic, sample-efficient stability certification algorithm (SCA) that yields non-trivial and interpretable guarantees for any attribution method. Moreover, we show that mild smoothing achieves a more favorable trade-off between accuracy and stability, avoiding the aggressive compromises made in prior certification methods. To explain this behavior, we use Boolean function analysis to derive a novel characterization of stability under smoothing. We evaluate SCA on vision and language tasks and demonstrate the effectiveness of soft stability in measuring the robustness of explanation methods.

==> figures/smoothing_frequency_shift_example.tex <==
\begin{figure}[t]
\centering

\includegraphics[width=1.0\linewidth]{images/example_spectrum.png}

\caption{
Smoothing shifts mass towards lower-order terms and decays the spectrum tail.
We sample a random weights \(\widehat{h}(S) \sim \mcal{N}(0, 1)\) and \(\widehat{g}(S) = \abs{\widehat{h}}(S)\).
(Left) The average \(\abs{\widehat{M_\lambda h}(S)}\) at each degree \(\abs{S} = k\), for \(k = 0, 1, \ldots, n\).
(Right) The average \(\abs{\widehat{M_\lambda g}(S)}\) at each \(\abs{S} = k\).
At \(\lambda = 1\) are the original weights.
}
\label{fig:smoothing_frequency_shift_example}
\end{figure}


==> neurips_checklist.tex <==

\newpage
\section*{NeurIPS Paper Checklist}

%%% BEGIN INSTRUCTIONS %%%
The checklist is designed to encourage best practices for responsible machine learning research, addressing issues of reproducibility, transparency, research ethics, and societal impact. Do not remove the checklist: {\bf The papers not including the checklist will be desk rejected.} The checklist should follow the references and follow the (optional) supplemental material.  The checklist does NOT count towards the page
limit. 

Please read the checklist guidelines carefully for information on how to answer these questions. For each question in the checklist:
\begin{itemize}
    \item You should answer \answerYes{}, \answerNo{}, or \answerNA{}.
    \item \answerNA{} means either that the question is Not Applicable for that particular paper or the relevant information is Not Available.
    \item Please provide a short (1–2 sentence) justification right after your answer (even for NA). 
   % \item {\bf The papers not including the checklist will be desk rejected.}
\end{itemize}

{\bf The checklist answers are an integral part of your paper submission.} They are visible to the reviewers, area chairs, senior area chairs, and ethics reviewers. You will be asked to also include it (after eventual revisions) with the final version of your paper, and its final version will be published with the paper.

The reviewers of your paper will be asked to use the checklist as one of the factors in their evaluation. While "\answerYes{}" is generally preferable to "\answerNo{}", it is perfectly acceptable to answer "\answerNo{}" provided a proper justification is given (e.g., "error bars are not reported because it would be too computationally expensive" or "we were unable to find the license for the dataset we used"). In general, answering "\answerNo{}" or "\answerNA{}" is not grounds for rejection. While the questions are phrased in a binary way, we acknowledge that the true answer is often more nuanced, so please just use your best judgment and write a justification to elaborate. All supporting evidence can appear either in the main paper or the supplemental material, provided in appendix. If you answer \answerYes{} to a question, in the justification please point to the section(s) where related material for the question can be found.

IMPORTANT, please:
\begin{itemize}
    \item {\bf Delete this instruction block, but keep the section heading ``NeurIPS Paper Checklist"},
    \item  {\bf Keep the checklist subsection headings, questions/answers and guidelines below.}
    \item {\bf Do not modify the questions and only use the provided macros for your answers}.
\end{itemize} 
 

%%% END INSTRUCTIONS %%%


\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We support our claims with both theoretical proofs and experimental evaluations.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A No or NA answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We discuss the limitations in~\cref{sec:additional_discussion}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper has no limitation while the answer No means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate "Limitations" section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory assumptions and proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We give some proofs of our claims in the main paper, as well as more in-depth treatment in~\cref{sec:standard_analysis} and~\cref{sec:monotone_analysis}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

    \item {\bf Experimental result reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We describe our experimental setup in~\cref{sec:experiments} and~\cref{sec:additional_experiments}.
    Moreover, we will make our code available open source when it is okay to do so.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item If the paper includes experiments, a No answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and/or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We will make our code available as open source when permitted to do so.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so “No” is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental setting/details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer, etc.) necessary to understand the results?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We give detailed descriptions of experiment setup in~\cref{sec:experiments} and~\cref{sec:additional_experiments}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment statistical significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We report error bars where appropriate.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The authors should answer "Yes" if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g. negative error rates).
        \item If error bars are reported in tables or plots, The authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments compute resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We describe compute resources in~\cref{sec:additional_experiments}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code of ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: To the best of our ability and knowledge, we have conformed to the NeurIPS Code of Ethics.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer No, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We discuss broader impacts in~\cref{sec:additional_discussion}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that there is no societal impact of the work performed.
        \item If the authors answer NA or No, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pretrained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We do not release new models and data.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: All assets are properly credited in the paper.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We do not introduce new assets in the paper.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset/code/model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and research with human subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We do not conduct research with human subjects.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional review board (IRB) approvals or equivalent for research with human subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We do not have human participants.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\item {\bf Declaration of LLM usage}
    \item[] Question: Does the paper describe the usage of LLMs if it is an important, original, or non-standard component of the core methods in this research? Note that if the LLM is used only for writing, editing, or formatting purposes and does not impact the core methodology, scientific rigorousness, or originality of the research, declaration is not required.
    %this research? 
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We used an LLM, RoBERTa, only for evaluating the stability of explanation methods.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the core method development in this research does not involve LLMs as any important, original, or non-standard components.
        \item Please refer to our LLM policy (\url{https://neurips.cc/Conferences/2025/LLM}) for what should or should not be described.
    \end{itemize}

\end{enumerate}


==> old/algorithm.tex <==
\begin{algorithm} [ht!]
\caption{Approximate Soft Stability Rate ($f, x, \alpha, r, \epsilon, \delta$)}\label{alg:approx_soft_stability_radii}
\begin{algorithmic}
    \STATE Set $N = \frac{\log(r/\delta)}{2\epsilon^2}$, where radius $r > 0$, tolerance $\epsilon > 0$, probability $\delta > 0$. \COMMENT{\red{XXX=XX} is sufficient.} \\
    \FOR{$k=1$ to $r$}
    \FOR{$i$ = 1 to $N$}
        \STATE Pick $\alpha_i^{(k)} \sim \Delta^{(k)}(\alpha).$
        \STATE Set $v_i \gets \mathbf{1}[f(x \odot \alpha_i^{(k)}) \cong f(x \odot \alpha)]$. \COMMENT{$v_i$ is 1 if $f(x \odot \alpha_i^{(k)}) \cong f(x \odot \alpha)$, 0 otherwise.}
    \ENDFOR
    \STATE Let $\hat{\mu}^{(k)} = \frac{1}{N}\sum_{i=1}^N v_i$ be the estimated frequency where $\alpha$ is stable after adding $k$ features.
    \ENDFOR{}
    \STATE Let $\hat{\tau}_r = \min_{k \leq r} \hat{\mu}^{(k)}$
\end{algorithmic}
\end{algorithm}

% \begin{algorithm} [ht!]
% \caption{Approximate Influence ($\epsilon, \gamma, \delta, S$) (\citep{levi2020tolerant})}\label{alg:approx_influence}
% \begin{algorithmic}
%     \STATE Set $m = \frac{C \cdot \ln(2/\delta)}{\gamma^2 \epsilon}$, where $C \geq 1$ is an absolute constant.  \COMMENT{$C \geq 3$ is sufficient.} \\
%     \FOR{$i$ = 1 to $m$}
%         \STATE Pick $x \sim \{0, 1\}^{\bar{S}}, u,v \sim \ \{0, 1\}^S$ uniformly at random and independently.
%         \STATE Set $v_i \in \mathds{1} \{ g(x \sqcup u) \neq g(x \sqcup v) \}$.  \COMMENT{$v_i$ is 1 if $g(x \sqcup u) \neq g(x \sqcup v)$, 0 otherwise.}
%     \ENDFOR \\
%     \STATE Let $\widetilde{\textbf{Inf}}_g (S) \gets \frac{2}{m} \sum_{i \in [m]} v_i$ be the estimate of the influence of $S$. 
%     % \Comment Note that in practice, we set $m$, the number of random samples or trials we take at each $k$, to be at least 50 due to law of large numbers.
% \end{algorithmic}
% \end{algorithm}

==> old/bound_proof.tex <==


\begin{lemma}
Consider any \(h: \{0,1\}^n \to \{0,1\}\).
Fix a tolerance \(\varepsilon > 0\), failure rate \(\delta > 0\), and integer \(k_{\msf{max}} > 0\).
For each \(k = 1, \ldots, k_{\msf{max}}\), sample:
\begin{equation*}
    \hat{\mu}^{(k)} = \frac{1}{N} \bracks*{ h(\alpha_1 ^{(k)}) + \cdots + h(\alpha_N ^{(k)})},
\end{equation*}
where each \(\alpha_i ^{(k)} \sim \{0,1\}^n\) with \(\abs{\alpha_i ^{(k)}} = k\), uniformly.
If there are \(N \geq \log(k_{\msf{max}} / \delta) / (2 \varepsilon^2)\)
samples for each \(\hat{\mu}^{(k)}\), then
\begin{equation*}
    \mrm{Pr}\bracks*{\bigcap_k \parens*{\mu^{(k)} > \tau}} \geq 1 - \delta,
\end{equation*}
where \(\mu^{(k)} = \mathbb{E}_{\alpha^{(k)}} [h(\alpha^{(k)})]\) and \(\tau = \min_k \hat{\mu}^{(k)} - \varepsilon\).
\end{lemma}
\begin{proof}
It suffices to show that
\begin{equation*}
    1 - \mrm{Pr}\bracks*{\bigcap_k \parens*{\mu^{(k)} > \tau}}
    = \mrm{Pr}\bracks*{\bigcup_k \parens*{\mu^{(k)} \leq \tau}}
    \leq \delta.
\end{equation*}
This holds by the union bound because for each \(k\):
\begin{align*}
    \mrm{Pr}\bracks*{\mu^{(k)} \leq \tau}
    &= \mrm{Pr}\bracks*{\mu^{(k)} \leq \min_j \hat{\mu}^{(j)} - \varepsilon} \\
    &\leq \mrm{Pr}\bracks*{\mu^{(k)} \leq \hat{\mu}^{(k)} - \varepsilon} \\
    &\leq \exp\parens*{-2\varepsilon^2 N}
        \tag{Hoeffding} \\
    &\leq \delta / k_{\msf{max}}.
    \tag{By our choice of \(N\)}
\end{align*}
\end{proof}


==> old/certificates_1.tex <==
\section{Certifying Soft Stability for Any Classifier}

We first discuss the limitations of existing methods of hard stability.
We then present a sampling algorithm with which one may certify the stability rate for any model.
Moreover, we present a smoothing algorithm called BISE, which is inspired by Boolean analysis, such that the stability rate of a BISE-smoothed classifier is improved.
We emphasize that one can certify the stability rate for both BISE-smoothed and non-BISE-smoothed classifiers.



\subsection{Limitations of Certifying Hard Stability}
\label{sec:limitations_of_hard_stability}

Existing methods certify hard stability by using a classifier's Lipschitz constant, which is a measure of global smoothness.
However, a classifier's Lipschitz constant is not known in general and is often computationally intractable to find.
The main idea in~\citet{xue2024stability} is to derive a classifier for which the Lipschitz constant is known by construction.
Starting with any pre-trained or readily available \textit{base classifier} \(g\), one defines the \textit{smoothed classifier} \(f\) as follows:
\begin{equation*}
    f(x) = \frac{1}{N} \bracks*{g(x ^{(1)}) + \cdots + g(x ^{(N)})},
    % \enskip
    % x_1 ', \ldots, x_N ' \sim \mcal{D}(x, \lambda),
\end{equation*}
where \(x^{(1)}, \ldots, x^{(N)} \sim \mcal{D}(x, \lambda)\) are carefully constructed perturbations of \(x\) parametrized by a real-valued constant \(\lambda > 0\).
If done correctly, \(f\) will have a Lipschitz constant of \(\lambda\), wherein a smaller \(\lambda\) means a smoother \(f\).
Because \(\lambda\) is known by construction, it can be used to yield stability guarantees for \(f\) at any input \(x\) and explanation \(\alpha\).
In particular, the general relation is as follows:
\begin{equation} %\label{eqn:smoothness_vs_cert_radius}
    % \text{Smoothness of \(f\)}
    \text{Smoothness}(f)
    % \propto
    \sim
    \text{CertifiableRadius}(f, x, \alpha)
    % \text{Certifiable Radius of \(\alpha\) at \(x\)}
\end{equation}
That is, the smoother the \(f\), the further distance from \(\alpha\) that we can certify up to.
However, this smoothness is in tension with the performance of \(f\):
\begin{equation*} %\label{eqn:smoothness_vs_accuracy}
    % \text{Smoothness of \(f\)}
    \text{Smoothness}(f)
    % \propto
    \sim
    - \text{Accuracy}(f)
    % - \text{Accuracy of \(f\)}
    % \frac{1}{\text{Accuracy of \(f\)}}
\end{equation*}
That is, using a smaller \(\lambda\) to construct \(\mcal{D}(x, \lambda)\) will result in a smoother \(f\), albeit one that performs worse.


The main reason for this tension is that the Lipschitz constant is a global measure of smoothness for \(f\).
By having a smoother \(f\), i.e., a classifier whose output landscape is ``flatter'', one can make more aggressive guarantees about how the output will change for different \(\alpha'\).
However, the Lipschitz constant \(\lambda\) is inversely correlated with the expressiveness of a function class, which means that smoother \(f\) are theoretically expected to perform worse, no matter the quality of the base classifier \(g\).


% The main reason for this trade-off between smoothness 

% The main reason for the tension between~\cref{eqn:smoothness_vs_cert_radius} and~\cref{eqn:smoothness_vs_accuracy} is because the Lipschitz constant is a global measure of smoothness for \(f\).






% \red{(There needs to be a very short description of the MuS algorithm)}


% To certify incremental stability,~\citet{xue2024stability} observe that when \(f\) satisfies a technical condition known as \textit{Lipschitz with respect to the masking of features}, then incremental stability can be certified in constant time.
% The key technical contribution is to present a sample-efficient, de-randomized smoothing algorithm known as \textit{Multiplicative Smoothing (MuS)}, which can turn any classifier \(g\) into a Lipschitz-smooth \(f\).

% \begin{theorem}[MuS, informal~\citet{xue2024stability}]
% Suppose that the classifier \(f: \mbb{R}^n \to [0,1]^m\) is \(\lambda\)-Lipschitz with respect to the masking of features.
% Let \(\alpha\) be an explanation for \(x\) on \(f\), then
% \begin{equation*}
%     r_{\msf{cert}} = \frac{f(x \odot \alpha)_{k_1} - f(x \odot \alpha)_{k_2}}{2 \lambda},
% \end{equation*}
% where \(k_1\) and \(k_2\) are the top-1 and top-2 classes of \(f(x \odot \alpha)\).
% \end{theorem}

% The main drawback of this is that we can only certify the stability for Lipschitz-smooth classifiers, which can have a trade-off in performance compared to non-smoothed classifiers.



\subsection{Probabilistic Guarantees for Soft Stability}


We now present an algorithm for certifying the soft stability \(\tau_r\) by measuring the stability rate of an explanation.
Because the true \(\tau_r\) is computationally intractable to measure, our approach is to do lots of sampling to get an estimation \(\hat{\tau}_r\) that is concentrated near the true value.
This algorithm and its guarantees are outlined in the following theorem.


\begin{theorem}[Sampling Algorithm]
Consider any tolerance \(\varepsilon > 0\), failure probability \(\delta > 0\), and sample size \(N \geq \log(1/\delta) / (2 \varepsilon^2)\).
For any classifier \(f\), input \(x\), explanation \(\alpha\), and radius \(r > 0\), let:
\begin{equation*}
    \hat{\tau}_r
    = \frac{1}{N} \sum_{i = 1}^{N} \mbf{1}\bracks*{f(x \odot \alpha^{(i)}) \cong f(x \odot \alpha)},
\end{equation*}
where each \(\alpha^{(i)} \sim \Delta_r\).
Then, \(\Pr{}\bracks{\tau_r \geq \hat{\tau_r} - \varepsilon} \geq 1 - \delta\).
\end{theorem}
\begin{proof}
This follows from using a one-sided Hoeffding's inequality to approximate the mean of Bernoulli random variables \(X^{(1)}, \ldots, X^{(N)}\), where
% \(X^{(i)} = \mbf{1}[f(x \odot \alpha^{(i)}) \cong f(x \odot \alpha)]\).
\begin{equation*}
    X^{(i)} = \mbf{1}[f(x \odot \alpha^{(i)}) \cong f(x \odot \alpha)].
\end{equation*}
\end{proof}

\red{AAAAAAAAAAAAAA}



\begin{theorem}
% \label{thm:sampling_stability_rate}
Consider any classifier \(f\), input \(x\), and explanation \(\alpha\).
Fix any radius \(r > 0\), tolerance \(\varepsilon > 0\), and failure probability \(\delta > 0\).
Using \(N \geq \log(r/\delta) / (2 \varepsilon^2)\) samples for each \(k = 1, \ldots, r\), let
\begin{equation*}
    \hat{\mu}^{(k)} = \frac{1}{N} \sum_{i = 1}^{N} \mbf{1}\bracks*{f(x \odot \alpha_i ^{(k)}) \cong f(x \odot \alpha)},
\end{equation*}
where \(\alpha_i ^{(k)} \sim \Delta^{(k)}\) uniformly.
Let \(\hat{\tau}_r = \min_{k\leq r} \hat{\mu}^{(k)}\), then
\begin{equation*}
    \prob{}\bracks*{
        \tau_r \geq \hat{\tau}_r - \varepsilon
    } \geq 1 - \delta.
\end{equation*}
\end{theorem}
\begin{proof}
This follows from~\cref{lem:stability_rate_lemma} if we take \(p = n - \abs{\alpha}\) and define the \(h: \{0,1\}^p \to \{0,1\}\) therein as:
\begin{equation*}
    h(\beta) = \mbf{1} \bracks*{f(x \odot (\alpha + \bar{\beta})) \cong f(x \odot \alpha)},
\end{equation*}
where \(\bar{\beta} \in \{0,1\}^n\) is the ``embedding'' of \(\beta \in \{0,1\}^p\).
\end{proof}

\input{icml2025/figures/algorithm}

\input{icml2025/figures/algorithm_fig}

We give an illustration of this algorithm in Figure~\ref{fig:algorithm_fig} and Algorithm~\ref{alg:approx_soft_stability_radii}.
Note that the guarantees obtainable in this manner are probabilistic, which is in contrast from those for hard stability.


\subsection{Further Improving Soft Stability with BISE}

While our results in the previous section applies to any classifier, we present a method for preprocessing classifiers, inspired by smoothing techniques from Boolean analysis, to improve the guarantees attainable by the above.


Using ideas from randomized smoothing, we further define another ...


\red{(Anton: this is some idea that I'd like to cook up to make the theory more ``impressive''. It's not strictly necessary for the paper story, but it would make things sound better + feel more complete.)}



\begin{definition}[BISE]
Let \(g: \mbb{R}^n \to \mbb{R}^m\) be any classifier.
For any \(0 \leq \rho \leq 1\), define the smoothing operator \(\mcal{S}_\rho\) by:
\begin{equation*}
    \mcal{S}_\rho g (x) = \expval{\beta \sim N_\rho} g(x \odot \beta)
\end{equation*}
\end{definition}


\citep{o2014analysis}


\red{Anton: I think there's a general plan that could go like this.
(1) Boolean functions that are ``low-degree'' have better stability rates ... for some reason.
(2) Smoothing lowers the ``degree'' of Boolean functions.
}


==> old/conclusion.tex <==
\section{Conclusion}

% We introduce soft stability, a probabilistic relaxation of hard stability that provides a more flexible and efficient way to certify the robustness of feature attributions.
% Unlike hard stability, soft stability is model-agnostic, sample-efficient, and does not require destructively modifying the classifier.
% Interestingly, we show that mild smoothing can improve the soft stability certificate of classifiers while incurring only a small cost to accuracy.
% We study this phenomenon from the perspective of Boolean function analysis and present novel characterizations and techniques that would be of interest to explainability researchers.
% Furthermore, we validate our theory through experiments on vision and language tasks.


We introduce soft stability, a probabilistic relaxation of hard stability that enables a more flexible and fine-grained measure of explanation robustness.
To certify soft stability, we introduce the Stability Certification Algorithm (SCA), a simple, model-agnostic, sampling-based algorithm that provides rigorous statistical guarantees that also extends to certifying hard stability.
Empirically, we demonstrate that SCA yields stronger stability guarantees than smoothing-based certification methods, such as MuS.
Although SCA does not require smoothing, we find that applying mild smoothing can further improve stability without significantly affecting accuracy.
To study this effect, we used Boolean analytic tooling to characterize stability under smoothing.
Finally, we validate our theory through experiments on vision and language models across a range of feature attribution methods.



==> old/hard_all_by_method.tex <==
\begin{figure*}[t]
\centering

\begin{minipage}{0.24\textwidth}
    \centering
    \includegraphics[width=\linewidth]{images/hard_vs_method_vit_imagenet_2_per_class_lime.pdf}
\end{minipage}\hfill
\begin{minipage}{0.24\textwidth}
    \centering
    \includegraphics[width=\linewidth]{images/hard_vs_method_resnet50_imagenet_2_per_class_lime.pdf}
\end{minipage}\hfill
\begin{minipage}{0.24\textwidth}
    \centering
    \includegraphics[width=\linewidth]{images/hard_vs_method_resnet18_imagenet_2_per_class_lime.pdf}
\end{minipage}\hfill
\begin{minipage}{0.24\textwidth}
    \centering
    \includegraphics[width=\linewidth]{images/hard_vs_method_roberta_tweeteval_all_lime.pdf}
\end{minipage}


\begin{minipage}{0.24\textwidth}
    \centering
    \includegraphics[width=\linewidth]{images/hard_vs_method_vit_imagenet_2_per_class_shap.pdf}
\end{minipage}\hfill
\begin{minipage}{0.24\textwidth}
    \centering
    \includegraphics[width=\linewidth]{images/hard_vs_method_resnet50_imagenet_2_per_class_shap.pdf}
\end{minipage}\hfill
\begin{minipage}{0.24\textwidth}
    \centering
    \includegraphics[width=\linewidth]{images/hard_vs_method_resnet18_imagenet_2_per_class_shap.pdf}
\end{minipage}\hfill
\begin{minipage}{0.24\textwidth}
    \centering
    \includegraphics[width=\linewidth]{images/hard_vs_method_roberta_tweeteval_all_shap.pdf}
\end{minipage}


\begin{minipage}{0.24\textwidth}
    \centering
    \includegraphics[width=\linewidth]{images/hard_vs_method_vit_imagenet_2_per_class_intgrad.pdf}
\end{minipage}\hfill
\begin{minipage}{0.24\textwidth}
    \centering
    \includegraphics[width=\linewidth]{images/hard_vs_method_resnet50_imagenet_2_per_class_intgrad.pdf}
\end{minipage}\hfill
\begin{minipage}{0.24\textwidth}
    \centering
    \includegraphics[width=\linewidth]{images/hard_vs_method_resnet18_imagenet_2_per_class_intgrad.pdf}
\end{minipage}\hfill
\begin{minipage}{0.24\textwidth}
    \centering
    \includegraphics[width=\linewidth]{images/hard_vs_method_roberta_tweeteval_all_intgrad.pdf}
\end{minipage}


\begin{minipage}{0.24\textwidth}
    \centering
    \includegraphics[width=\linewidth]{images/hard_vs_method_vit_imagenet_2_per_class_mfaba.pdf}
\end{minipage}\hfill
\begin{minipage}{0.24\textwidth}
    \centering
    \includegraphics[width=\linewidth]{images/hard_vs_method_resnet50_imagenet_2_per_class_mfaba.pdf}
\end{minipage}\hfill
\begin{minipage}{0.24\textwidth}
    \centering
    \includegraphics[width=\linewidth]{images/hard_vs_method_resnet18_imagenet_2_per_class_mfaba.pdf}
\end{minipage}\hfill
\begin{minipage}{0.24\textwidth}
    \centering
    \includegraphics[width=\linewidth]{images/hard_vs_method_roberta_tweeteval_all_mfaba.pdf}
\end{minipage}


\begin{minipage}{0.24\textwidth}
    \centering
    \includegraphics[width=\linewidth]{images/hard_vs_method_vit_imagenet_2_per_class_random.pdf}
\end{minipage}\hfill
\begin{minipage}{0.24\textwidth}
    \centering
    \includegraphics[width=\linewidth]{images/hard_vs_method_resnet50_imagenet_2_per_class_random.pdf}
\end{minipage}\hfill
\begin{minipage}{0.24\textwidth}
    \centering
    \includegraphics[width=\linewidth]{images/hard_vs_method_resnet18_imagenet_2_per_class_random.pdf}
\end{minipage}\hfill
\begin{minipage}{0.24\textwidth}
    \centering
    \includegraphics[width=\linewidth]{images/hard_vs_method_roberta_tweeteval_all_random.pdf}
\end{minipage}




\caption{
\textbf{Hard stability certificates, by explanation methods.}
At any smoothing parameter \(\lambda\), the maximum certifiable hard stability radius is only \(1 / 2\lambda\) by~\cref{thm:hard_stability_radius}.
}
\label{fig:hard_all_by_method}
\end{figure*}


==> old/hard_stability_rates_varying_lambda_roberta.tex <==
\begin{figure*}[t]
\centering
\begin{minipage}{0.31\textwidth}
    \centering
    \includegraphics[width=\linewidth]{images/roberta_tweeteval_lime_hard_varying_lambda.pdf}
\end{minipage}
\quad
\begin{minipage}{0.31\textwidth}
    \centering
    \includegraphics[width=\linewidth]{images/roberta_tweeteval_shap_hard_varying_lambda.pdf}
\end{minipage}
\quad
\begin{minipage}{0.31\textwidth}
    \centering
    \includegraphics[width=\linewidth]{images/roberta_tweeteval_intgrad_hard_varying_lambda.pdf}
\end{minipage}
\quad
\begin{minipage}{0.31\textwidth}
    \centering
    \includegraphics[width=\linewidth]{images/roberta_tweeteval_mfaba_hard_varying_lambda.pdf}
\end{minipage}
\quad
\begin{minipage}{0.31\textwidth}
    \centering
    \includegraphics[width=\linewidth]{images/roberta_tweeteval_random_hard_varying_lambda.pdf}
\end{minipage}

\caption{
\textbf{(RoBERTa) Hard stability rates for varying lambda parameters.}
We show the hard stability rates for different explanation methods at different values of \(\lambda = 0.125, 0.25, 0.5\).
}
\label{fig:hard_stability_rates_varying_lambda_roberta}
\end{figure*}


==> old/initial_feature_sizes.tex <==
\begin{figure}[t]
\centering

\begin{minipage}{0.48\linewidth}
    \centering
    \includegraphics[width=1.0\linewidth]{images/resnet18_plusr20_stability_vs_asize.pdf}
\end{minipage}
\hfill
\begin{minipage}{0.48\linewidth}
    \centering
    \includegraphics[width=1.0\linewidth]{images/resnet18_plusr40_stability_vs_asize.pdf}
\end{minipage}

\caption{
\textbf{Larger initial feature selections lead to higher stability rates, which improve with greater smoothing (smaller \(\lambda\)).}
(Left) Stability rates at perturbation radius \(r = 20\) for different initial selection sizes of \(\alpha\).
(Right) Stability rates at perturbation \(r = 40\).
% There are a total of \(196\) patches.
}
\label{fig:initial_feature_sizes}
\end{figure}

==> old/introduction_1.tex <==


\section{Introduction}


Powerful machine learning models are increasingly deployed in practice.
However, their opacity presents a major challenge in being adopted in high-stake domains, where transparent explanations are needed in decision making.
In healthcare, for instance, doctors require insights into the diagnostic steps to trust the model and integrate them into clinical practice effectively~\citep{klauschen2024toward}.
Similarly, in the legal domain, attorneys must ensure that decisions reached with the assistance of models meet stringent judicial standards~\citep{richmond2024explainable}.


% \input{figures/intro_non_stable_example}


There is much interest in explaining the behavior of complex models.
One popular class of explanation methods are \textit{feature attributions}~\citep{ribeiro2016should,lundberg2017unified}, which aim to identify the most important input features that contribute to a model's prediction.
However, many explanations are \textit{unstable}, as illustrated in~\cref{fig:intro_non_stable_example}: additionally revealing some features will change the model's prediction.
This kind of non-robustness is often undesirable because it suggests that the given explanation is unreliable~\citep{wagner2019interpretable,nauta2023anecdotal,yeh2019fidelity}.

% We show such an example in~\cref{fig:hard_stability_vs_soft_stability} using the features selected by LIME~\citep{ribeiro2016should}.
% A common way to evaluate an attribution method is to test whether the selected features contain enough information to recover the original prediction~\citep{wagner2019interpretable,nauta2023anecdotal}.
% The selection in this example can do so, but including a single additional patch can drastically alter the predicted label.
% Despite the complexity of modern classifiers, this behavior is often undesirable because it suggests that providing more information can paradoxically decrease the model's confidence~\citep{yeh2019fidelity}.




Such phenomenon has sparked interest in quantifying how model predictions vary with attributions, such as the effect of adding or removing features~\citep{wu2020towards,samek2016evaluating} and the impact of the selection's shape~\citep{hase2021out,rong2022consistent}.
However, most existing works focus on empirical measures~\citep{agarwal2022openxai}, with limited formal, mathematical guarantees on the robustness of attribution-induced predictions.


To address this gap, prior work in \citet{xue2024stability} consider \textit{stability} as a formal certification framework for feature selection.
In particular, a \textit{stable explanation} is one in which adding a small number of features does not alter the model's prediction, thereby eliminating the undesirable behavior illustrated in~\cref{fig:intro_non_stable_example}.
This property is quantified by its \textit{certified radius}, which measures the maximum number of additional features that can be included while preserving the prediction.


% \begin{center}
% \begin{minipage}{0.9\linewidth}
% A set of features is \textit{\textbf{stable}} if adding a few additional features does not change the induced prediction.
% \end{minipage}
% \end{center}


However, stability is not simple to certify.
If the classifier lacks favorable properties, one must exhaustively check predictions for all possible feature additions in a computationally intractable manner.
To overcome this, \citet{xue2024stability} apply smoothing techniques from the adversarial robustness~\citep{cohen2019certified,levine2021improved} to transform arbitrary models into \textit{smoothed classifiers} with convenient properties for efficiently computing certified radii.
In practice, however, these radii are often small and apply only to the smoothed classifier rather than the original model.
Furthermore, smoothing typically degrades a classifier's accuracy.
While these guarantees are meaningful, they remain conservative and impose a harsh accuracy trade-off on the smoothed classifier.



\input{figures/different_kinds_of_stability}


In this work, we present a new variant of stability that we call \textit{soft stability}.
We define this in contrast to that of~\citet{xue2024stability}, which we refer to as \textit{hard stability} from this point forward.
While hard stability certifies whether \textit{all} small perturbations to an attribution yield the same prediction, soft stability instead quantifies \textit{how often} the prediction remains consistent.
This is a probabilistic relaxation of hard stability that avoids the need to smooth the classifier.
In general, probabilistic guarantees are flexible to apply and efficient to compute compared to their hard variants.
Consequently, they have gained traction in machine learning applications such as medical imaging~\citep{fayyad2024empirical}, drug discovery~\citep{arvidsson2024cpsign}, and autonomous driving~\citep{lindemann2023safe}.
Conveniently, probabilistic guarantees are also often formulated in terms of \textit{confidence}, which is widely explored in machine learning and explainability literature~\citep{angelopoulos2023conformal,carvalho2019machine,atanasova2024diagnostic}.


In this work, we advance the understanding of robust feature-based explanations by extending probabilistic guarantees to stability.
Our analyses and experiments provide new insights into attribution robustness, especially on the role of smoothed classifiers.
Our key contributions are as follows.



% \paragraph{Soft Stability is Easy to Apply and Certify}
% \paragraph{Soft Stability is Model-Agnostic, Sample-Efficient, and Attains Useful Guarantees}
\paragraph{Soft Stability is Practical and Attains Useful Guarantees}
We introduce soft stability to address the limitations of hard stability.
Soft stability certification is model-agnostic and provides non-trivial guarantees that are practically interpretable.
In contrast, hard stability certification relies on heavily smoothed classifiers, which not only suffer from accuracy degradation but also yield overly conservative guarantees.
In~\cref{sec:certifying_soft_stability}, we examine the drawbacks of hard stability and introduce an efficient soft stability certification algorithm.



% Need to pose this as a result that we showed
% More like want to show that mild smoothing is sufficient
% Be more direct with it in the text: just say that you have created a state-of-the-art
% Just say it's up to two orders of magnitude ...
% "Have to sell even theory!" ~ riceric22


% Also need to set up that the theoretical problem is not solved yet, otherwise it's harder for people to understand why did the theory in the first place
% In this paoer, we formally show the connection and prove that ...

\paragraph{Mild Smoothing Improves Soft Stability}
Although soft stability certification does not require smoothing, we found that mild smoothing can improve guarantees without incurring the severe accuracy degradation typically associated with the smoothing-based certification of hard stability.
To explain this phenomenon, we developed new techniques for analyzing the effects of smoothing on stability using Boolean function analysis.
We give an overview of our main theoretical results in~\cref{sec:smoothing}.


\paragraph{Soft Stability Outperforms Hard Stability}
We empirically validated the improvement of soft stability over hard stability on a combination of vision and language tasks and various feature attribution methods.
In particular, the attainable soft stability certificates are often two orders of magnitude stronger than the hard stability certificates.
Moreover, we show that mildly smoothed classifiers attain a good trade-off between accuracy and stability.
We present our experimental results in~\cref{sec:experiments}.



% We conduct experiments on vision and language tasks to validate our theoretical developments.
% Specifically, we compare the guarantees of soft and hard stability and analyze the effect of smoothing on classifier performance.
% These experiments provide empirical support for our claims and are detailed in~\cref{sec:experiments}.



==> old/monotone_analysis_1.tex <==
\section{Analysis of Stability and Smoothing in the Monotone Basis}
\label{sec:stability_via_monotone_basis}


The analysis of feature attribution stability naturally leads to studying Boolean functions under one-way perturbations. While Fourier analysis is the standard tool for Boolean function analysis, it has key limitations for our setting. First, it treats 0→1 and 1→0 transitions symmetrically, making it harder to analyze perturbations that only add features (\(\beta \geq \alpha\)) and smoothing operations that only remove features (via masking). Second, the traditional spectral analysis focuses on global properties, while our stability guarantees are inherently local (they depend on the specific attribution \(\alpha\)). This asymmetry in our setting, combined with our focus on mild smoothing (\(\lambda \approx 1\)), motivates the development of new analytical tools.

\subsection{Monotone Basis for Boolean Functions}
To respect this one-way nature of perturbations, we introduce a monotone basis. For any set \(T \subseteq [n]\):
\begin{equation*}
    \mbf{1}_T(\alpha) = \begin{dcases}
        1 & \text{if } \alpha_i = 1 \text{ for all } i \in T \text{ (all features in \(T\) present)} \\
        0 & \text{otherwise (any feature in \(T\) absent)}
    \end{dcases}
\end{equation*}

Unlike the standard Fourier basis, the monotone basis is not orthonormal. However, it satisfies certain desirable properties:
\begin{lemma}
\label{lem:monotone_basis}
Any Boolean function \(h: \{0,1\}^n \to \mbb{R}\) can be uniquely expressed in the monotone basis:
\begin{equation*}
    h(\alpha) = \widetilde{h}(\emptyset) + \sum_{T \subseteq [n], T \neq \emptyset} \widetilde{h}(T) \mbf{1}_T(\alpha)
\end{equation*}
where \(\widetilde{h}(T)\) are the monotone basis coefficients of \(h\), \(\widetilde{h}(\emptyset)\) is a constant term, and \(\mbf{1}_\emptyset(\alpha) = 1\) for all \(\alpha\).
The basis functions satisfy:
\begin{equation*}
    \expval{\alpha \sim \{0,1\}^n}[\mbf{1}_S(\alpha)\mbf{1}_T(\alpha)] = 2^{-|S \cup T|}
\end{equation*}
and the coefficients can be computed recursively:
\begin{equation*}
    \widetilde{h}(T) = h(T) - \sum_{S \subsetneq T} \widetilde{h}(S)
\end{equation*}
where \(h(T)\) means evaluating \(h\) on the attribution with 1's exactly at positions in \(T\).
\end{lemma}

\begin{proof}[Proof of Lemma~\ref{lem:monotone_basis}]
First, we prove existence and uniqueness. For any attribution \(\alpha\), let \(S_\alpha = \{i: \alpha_i = 1\}\) be its support. By definition of \(\mbf{1}_T\):
\begin{align*}
    h(\alpha) &= \widetilde{h}(\emptyset) + \sum_{\substack{T \subseteq [n] \\ T \neq \emptyset}} \widetilde{h}(T) \mbf{1}_T(\alpha) \\
    &= \widetilde{h}(\emptyset) + \sum_{T \subseteq S_\alpha} \widetilde{h}(T) \tag{support restriction}
\end{align*}

This gives a system of \(2^n\) linear equations (one for each \(\alpha\)) in \(2^n\) unknowns (the coefficients \(\widetilde{h}(T)\)). When we order both attributions and sets by inclusion, for each set \(T\), all proper subsets \(S \subsetneq T\) appear before \(T\) in the ordering. This creates an upper triangular matrix with 1's on the diagonal (since \(\mbf{1}_T(T) = 1\) and \(\mbf{1}_T(S) = 0\) for \(|S| < |T|\)), proving existence and uniqueness.

For the inner product formula:
\begin{align*}
    \expval{\alpha}\bigl[\mbf{1}_S(\alpha)\mbf{1}_T(\alpha)\bigr] 
    &= \prob{\alpha}\bigl[\alpha_i = 1 \text{ for all } i \in S \cup T\bigr] \tag{product rule} \\
    &= 2^{-|S \cup T|} \tag{uniform distribution}
\end{align*}

For the recursive formula, fix a set \(T\) and consider \(h(T)\). By the expansion:
\begin{align*}
    h(T) &= \widetilde{h}(\emptyset) + \sum_{S \subseteq T} \widetilde{h}(S) \tag{basis expansion} \\
    &= \widetilde{h}(T) + \widetilde{h}(\emptyset) + \sum_{S \subsetneq T} \widetilde{h}(S) \tag{split largest term}
\end{align*}

Rearranging gives the recursive formula:
\begin{equation*}
    \widetilde{h}(T) = h(T) - \sum_{S \subsetneq T} \widetilde{h}(S) \tag{recursion}
\end{equation*}
\end{proof}

To build intuition for this basis, consider the following example:
\begin{example}[Conjunction vs Fourier]
\label{ex:conjunction}
Consider the conjunction of two features: \(h(\alpha) = \alpha_1 \land \alpha_2\). This function outputs 1 only when both features are present.
Recall that in the standard Fourier basis with \(\chi_T(\alpha) = (-1)^{|\supp(\alpha) \cap T|}\), we have:
\begin{equation*}
    h(\alpha) = \frac{1}{4} - \frac{1}{4}\chi_{\{1\}}(\alpha) - \frac{1}{4}\chi_{\{2\}}(\alpha) + \frac{1}{4}\chi_{\{1,2\}}(\alpha).
\end{equation*}
In the monotone basis, by contrast, this is simply
\(h(\alpha) = \mbf{1}_{\{1,2\}}(\alpha)\).
This directly captures the AND operation: the function is 1 exactly when both features are present.
\end{example}

\subsection{Connection between Stability and Monotone Basis Expansion}
We will focus on \(f: \mbb{R}^n \rightarrow \mbb{R}\) (binary classification) and consider the following notion of model prediction equivalence.
\begin{definition}[Model Prediction Equivalence]
For a classifier \(f: \mathcal{X} \to \mathcal{Y}\) and input \(x\), we say two predictions are equivalent, denoted \(f(x \odot \beta) \cong f(x \odot \alpha)\), if:
\begin{equation*}
    |f(x \odot \beta) - f(x \odot \alpha)| \leq 1/2
\end{equation*}
\end{definition}
For binary classifiers where \(\mathcal{Y} = \{0,1\}\), this means the predictions must be identical. For probabilistic classifiers where \(\mathcal{Y} = [0,1]\), this allows for small variations in confidence while preserving the predicted class.
The monotone basis let us derive tight bounds on both soft and hard stability. We begin with soft stability:

\begin{lemma}[Soft Stability]
\label{lem:soft_stability}
For any Boolean function \(h: \{0,1\}^n \to [0,1]\) and attribution \(\alpha\), the stability rate \(\tau_r\) satisfies:
\begin{equation*}
    1 - \tau_r \leq \frac{2}{\sum_{i=0}^r \binom{n-|\alpha|}{i}} \sum_{\substack{j=1 \\ S: |S|=j \\ S \cap \supp(\alpha) = \emptyset}}^r \left|\sum_{T \subseteq S \setminus \{\emptyset\}} \widetilde{h}(T)\right|
\end{equation*}
where \(\widetilde{h}(T)\) are the coefficients in the monotone basis.
\end{lemma}

\begin{proof}[Proof of Lemma~\ref{lem:soft_stability}]
We begin with the definition of stability rate. By Markov's inequality:
\begin{align*}
    1 - \tau_r &= \prob{\beta \sim \Delta_r(\alpha)}\bigl[|h(\beta) - h(\alpha)| > 1/2\bigr] \\
    &\leq 2\expval{\beta \sim \Delta_r(\alpha)}\bigl[|h(\beta) - h(\alpha)|\bigr] \tag{Markov}
\end{align*}

To analyze the difference \(h(\beta) - h(\alpha)\), we express it using the monotone basis:
\begin{align*}
    h(\beta) - h(\alpha) &= \sum_{T \subseteq [n]} \widetilde{h}(T)\bigl(\mbf{1}_T(\beta) - \mbf{1}_T(\alpha)\bigr)
\end{align*}

Since perturbations only add features (\(\beta \geq \alpha\)), the difference in indicator functions simplifies considerably.
In particular, we have for any set \(T\) that:
\begin{equation*}
    \mbf{1}_T(\beta) - \mbf{1}_T(\alpha) = 
    \begin{cases}
        1 & \text{if \(T \neq \emptyset\) and (\(\forall i \in T, \beta_i = 1\)) and (\(\exists j \in T, \alpha_j = 0\))}, \\
        0 & \text{otherwise}
    \end{cases}
\end{equation*}

This allows us to rewrite the difference as a sum over only the relevant sets:
\begin{align*}
    h(\beta) - h(\alpha) &= \sum_{T: \alpha_i = 0, \beta_i = 1 \text{ for all } i \in T \setminus \{\emptyset\}} \widetilde{h}(T)
\end{align*}

To compute the expectation of \(|h(\beta) - h(\alpha)|\), we first need to understand the structure of this difference for any fixed \(\beta\). Note that \(\beta\) is completely determined by the set of positions \(S\) where it differs from \(\alpha\) (where zeros become ones). By construction of \(\Delta_r(\alpha)\), this set \(S\) must satisfy two properties: \(|S|=j\) for some \(j \leq r\), and \(S \cap \supp(\alpha) = \emptyset\) since we can only flip zeros to ones.
For such a fixed set \(S\), we can simplify our expression for \(h(\beta) - h(\alpha)\):
\begin{equation*}
    h(\beta) - h(\alpha) = \sum_{T \subseteq S, T \neq \emptyset} \widetilde{h}(T)
\end{equation*}
This simplification follows because a set \(T\) contributes to the difference if and only if it is contained in \(S\) (the positions where \(\beta\) differs from \(\alpha\)).

Now we can compute the expectation by considering how \(\beta\) is sampled under \(\Delta_r(\alpha)\). The sampling process has two steps: first, choose the number of positions \(j \sim \{0, 1, \ldots, r\}\) to flip with probability proportional to \(\frac{\binom{n-|\alpha|}{j}}{\sum_{i=0}^r \binom{n-|\alpha|}{i}}\); then, uniformly select \(j\) positions from the zeros in \(\alpha\). This gives us:
\begin{align*}
    \expval{\beta}\bigl[|h(\beta) - h(\alpha)|\bigr] 
    &= \sum_{j=1}^r \sum_{\substack{S:|S|=j \\ S \cap \supp(\alpha) = \emptyset}} \frac{1}{\sum_{i=0}^r \binom{n-|\alpha|}{i}} \left|\sum_{T \subseteq S \setminus \{\emptyset\}} \widetilde{h}(T)\right|
\end{align*}
Combining this with our initial Markov inequality bound completes the proof:
\begin{equation*}
    1 - \tau_r \leq \frac{2}{\sum_{i=1}^r \binom{n-|\alpha|}{i}} \sum_{\substack{j=1 \\ S: |S|=j \\ S \cap \supp(\alpha) = \emptyset}}^r \left|\sum_{T \subseteq S \setminus \{\emptyset\}} \widetilde{h}(T)\right|
\end{equation*}
\end{proof}

Here we present a simplification of the soft-stability bound above to make it easier to parse.
\begin{lemma}[Simplified Soft Stability Bound]
Under the same conditions, we also have:
\begin{equation*}
    1 - \tau_r \leq 2\sum_{k=1}^r \sum_{\substack{T: |T|=k \\ T \cap \supp(\alpha) = \emptyset}} |\widetilde{h}(T)| \cdot \frac{\sum_{j=k}^r \binom{n-|\alpha|-k}{j-k}}{\sum_{j=0}^r \binom{n-|\alpha|}{i}}
\end{equation*}
\end{lemma}
\begin{proof}
Starting from the bound in Lemma~\ref{lem:soft_stability}:
\begin{align*}
    1 - \tau_r &\leq \frac{2}{\sum_{i=0}^r \binom{n-|\alpha|}{i}} \sum_{j=1}^r \sum_{\substack{S:|S|=j \\ S \cap \supp(\alpha) = \emptyset}} \biggl|\sum_{T \subseteq S \setminus \{\emptyset\}} \widetilde{h}(T)\biggr| \\
    &\leq \frac{2}{\sum_{i=0}^r \binom{n-|\alpha|}{i}} \sum_{j=1}^r \sum_{\substack{S:|S|=j \\ S \cap \supp(\alpha) = \emptyset}} \sum_{T \subseteq S \setminus \{\emptyset\}} |\widetilde{h}(T)| \tag{triangle inequality} \\
    &= \frac{2}{\sum_{i=0}^r \binom{n-|\alpha|}{i}} \sum_{k=1}^r \sum_{\substack{T:|T|=k \\ T \cap \supp(\alpha) = \emptyset}} |\widetilde{h}(T)| \sum_{j=k}^r \binom{n-|\alpha|-k}{j-k} \tag{reorder sums} \\
    &= 2\sum_{k=1}^r \sum_{\substack{T:|T|=k \\ T \cap \supp(\alpha) = \emptyset}} |\widetilde{h}(T)| \cdot \frac{\sum_{j=k}^r \binom{n-|\alpha|-k}{j-k}}{\sum_{j=0}^r \binom{n-|\alpha|}{i}} \tag{rearrange}
\end{align*}

The derivation proceeds in three steps. We begin by applying the triangle inequality to separate the coefficients. Next, we reorder the summation to group terms by coefficient size. Finally, we count the occurrences of each coefficient in the sum. The final expression weights each coefficient \(\widetilde{h}(T)\) by \(\frac{\sum_{j=k}^r \binom{n-|\alpha|-k}{j-k}}{\sum_{j=0}^r \binom{n-|\alpha|}{i}}\), which is the probability that a random perturbation contains set \(T\) of size \(k\).
\end{proof}

Observe that the bound depends only on the monotone expansion terms of degree \(\le r\).
We can use the same technique above to derive a hard stability bound in terms of the monomial expansion as well.

\begin{lemma}[Hard Stability Bound]
For any Boolean function \(h: \{0,1\}^n \to [0,1]\) and attribution \(\alpha\), let
\begin{equation*}
    r^* = \max\left\{r \geq 0: \max_{\substack{S \subseteq [n] \\ 1 \leq |S| \leq r \\ S \cap \supp(\alpha) = \emptyset}} \left|\sum_{T \subseteq S \setminus \{\emptyset\}} \widetilde{h}(T)\right| \leq \frac{1}{2}\right\}
\end{equation*}
Then \(h\) is hard-stable at radius \(r^*\). 
\end{lemma}

\begin{proof}
For any \(\beta \in \Delta_r(\alpha)\):
\begin{align*}
    |h(\beta) - h(\alpha)| &= \left|\sum_{T \subseteq \text{diff}(\beta,\alpha) \setminus \{\emptyset\}} \widetilde{h}(T)\right|
\end{align*}
since \(\text{diff}(\beta,\alpha)\) is always a non-empty subset of size at most \(r\) disjoint from \(\supp(\alpha)\). By definition of \(r^*\), \(|h(\beta) - h(\alpha)| \leq 1/2\) for all \(\beta \in \Delta_{r^*}(\alpha)\), proving hard stability.
\end{proof}

\subsection{Stability Bound for Smoothed Distribution}
The monotone basis allows us to capture random masking as a simple transformation.

\begin{theorem}[Smoothing in Monotone Basis]
\label{thm:smoothing}
Let \(M_\lambda\) be the smoothing operator that randomly masks features with probability \(1-\lambda\):
\begin{equation*}
    M_\lambda h(\alpha) = \expval{z \sim \msf{Bern}(\lambda)^n}\bigl[h(\alpha \odot z)\bigr]
\end{equation*}
where \(z\) represents a random mask and \(\odot\) denotes element-wise multiplication as defined in~\cref{sec:basic_analysis_of_smoothing}.

For any Boolean function \(h: \{0,1\}^n \to [0,1]\), the smoothed function \(M_\lambda h\) in the monotone basis satisfies:
\begin{equation*}
    \widetilde{M_\lambda h}(T) = 
    \begin{cases}
        \widetilde{h}(\emptyset), & \text{if } T = \emptyset \text{ (constant term preserved)}, \\
        \lambda^{|T|} \widetilde{h}(T), & \text{if } T \neq \emptyset \text{ (coefficients damped)},
    \end{cases}
\end{equation*}
where \(\widetilde{M_\lambda h}(T)\) and \(\widetilde{h}(T)\) are the monotone basis coefficients of \(M_\lambda h\) and \(h\) respectively.
\end{theorem}

\begin{proof}[Proof of Theorem~\ref{thm:smoothing}]
First, note that \(M_\lambda\) is a linear operator since expectation is linear. For the empty set, \(\widetilde{M_\lambda h}(\emptyset) = \widetilde{h}(\emptyset)\) since smoothing preserves constants.

For any non-empty set \(T\):
\begin{align*}
    M_\lambda \mbf{1}_T(\alpha) &= \expval{z \sim \msf{Bern}(\lambda)^n}\bigl[\mbf{1}_T(\alpha \odot z)\bigr] \\
    &= \expval{z \sim \msf{Bern}(\lambda)^n}\biggl[\prod_{i \in T} (\alpha_i z_i)\biggr] \\
    &= \prod_{i \in T} \bigl(\alpha_i \expval{z_i \sim \msf{Bern}(\lambda)}[z_i]\bigr) \\
    &= \lambda^{|T|} \mbf{1}_T(\alpha)
\end{align*}
The result follows by linearity of expectation.
\end{proof}

With the above theorem in hand, we can now compute the stability of the smoothed classifier:
\begin{corollary}[Stability of Smoothed Functions]
\label{cor:smoothed_stability}
For any Boolean function \(h: \{0,1\}^n \to [0,1]\), attribution \(\alpha\), and smoothing parameter \(\lambda \in [0,1]\), the stability rate of the smoothed function satisfies:
\begin{equation*}
    1 - \tau_r(M_\lambda h) \leq 2\sum_{k=1}^r \lambda^k \sum_{\substack{T: |T|=k \\ T \cap \supp(\alpha) = \emptyset}} |\widetilde{h}(T)| \cdot \frac{\sum_{j=k}^r \binom{n-|\alpha|-k}{j-k}}{\sum_{j=0}^r \binom{n-|\alpha|}{i}}
\end{equation*}
This shows that smoothing improves stability by exponentially dampening the influence of larger feature sets.
\end{corollary}

\begin{proof}[Proof of Corollary~\ref{cor:smoothed_stability}]
Apply the stability bound from Lemma~\ref{lem:soft_stability} to \(M_\lambda h\) and use Theorem~\ref{thm:smoothing} which shows that \(\widetilde{M_\lambda h}(T) = \lambda^{|T|} \widetilde{h}(T)\) for non-empty \(T\):
\begin{align*}
    1 - \tau_r(M_\lambda h) &\leq 2\sum_{k=1}^r \sum_{\substack{T:|T|=k \\ T \cap \supp(\alpha) = \emptyset}} |\widetilde{M_\lambda h}(T)| \cdot \frac{\sum_{j=k}^r \binom{n-|\alpha|-k}{j-k}}{\sum_{j=0}^r \binom{n-|\alpha|}{i}} \tag{by Lemma~\ref{lem:soft_stability}} \\
    &= 2\sum_{k=1}^r \sum_{\substack{T:|T|=k \\ T \cap \supp(\alpha) = \emptyset}} \lambda^k|\widetilde{h}(T)| \cdot \frac{\sum_{j=k}^r \binom{n-|\alpha|-k}{j-k}}{\sum_{j=0}^r \binom{n-|\alpha|}{i}} \tag{by Theorem~\ref{thm:smoothing}} \\
    &= 2\sum_{k=1}^r \lambda^k \sum_{\substack{T:|T|=k \\ T \cap \supp(\alpha) = \emptyset}} |\widetilde{h}(T)| \cdot \frac{\sum_{j=k}^r \binom{n-|\alpha|-k}{j-k}}{\sum_{j=0}^r \binom{n-|\alpha|}{i}} \tag{rearrange terms}
\end{align*}

The final expression shows how smoothing affects stability through three key mechanisms. First, each coefficient \(\widetilde{h}(T)\) is weighted by \(\lambda^k\) where \(k = |T|\). Second, larger sets \(T\) are dampened more strongly since \(\lambda^k\) decreases exponentially with \(k\). Finally, the combinatorial terms \(\frac{\sum_{j=k}^r \binom{n-|\alpha|-k}{j-k}}{\sum_{j=0}^r \binom{n-|\alpha|}{i}}\) represent the probability of including set \(T\) in a random perturbation.
\end{proof}

\begin{remark}[Smoothing Effect]
\label{rem:smoothing}
The upper bound for the smoothed function in Corollary~\ref{cor:smoothed_stability} is at least a factor of \(\lambda\) smaller than the upper bound for the original function, since \(\lambda^k \leq \lambda\) for all \(k \geq 1\). However, these are only upper bounds - the actual improvement from smoothing could be either better or worse than suggested by comparing these bounds.
\end{remark}

\subsection{Discussion and Practical Implications}
Our analysis using a monotone basis reveals some key mechanisms affecting stability.
First, mild smoothing (\(\lambda \approx 1\)) can be effective because it exponentially dampens higher-order terms while preserving essential low-order structure --- for instance, with \(\lambda = 0.9\), single-feature terms are dampened by 0.9.
In comparison, five-feature terms are dampened by \(0.9^5 \approx 0.59\).
While our bounds guarantee at least a factor of \(\lambda\) improvement in stability (since \(\lambda^k \leq \lambda\) for all \(k \geq 1\)), the actual improvement could be either better or worse in practice.
Second, stability becomes harder to maintain at larger radii because both the number of terms and their combinatorial weights grow with \(r\), suggesting that \(\lambda\) should be chosen based on the distribution of \(|\widetilde{h}(T)|\) across different set sizes. 

While this work establishes the theoretical foundations, we could use these insights to design new attribution methods that explicitly control the monotone basis expansion of their output --- for instance, by regularizing higher-order coefficients or by constructing explanations primarily from small low-order terms. This suggests a new shift approach to attribution stability: rather than focusing solely on Lipschitz constants of the model, we should study the distribution of monotone basis coefficients, as these more directly capture the stability properties we care about.

==> old/notes_for_surbhi.tex <==
\section{\red{Hi Surbhi, here are some notes}}

A \(p\)-biased basis function \(\chi_S ^P\) on \(\{0,1\}^n\) is defined as
\begin{equation*}
    \chi_S ^p (\alpha) = \prod_{i \in S} \frac{p - \alpha_i}{\sigma_p},
    \quad \sigma_p = \sqrt{p (1 - p)},
\end{equation*}
where we immediately have:
\begin{align}
    \expval{\alpha_i \sim \Bern(p)} \frac{p - \alpha_i}{\sigma_p}
    &= p \parens*{\frac{p - 1}{\sigma_p}} + (1-p) \parens*{\frac{p}{\sigma_p}}
    = \frac{p^2 - p + p - p^2}{\sigma_p}
    = 0 \\
    \expval{\alpha_i \sim \Bern(p)} \parens*{\frac{p - \alpha_i}{\sigma_p}}^2
    &= p \parens*{\frac{p - 1}{\sigma_p}}^2
    + (1 - p) \parens*{\frac{p}{\sigma_p}}^2
    = \frac{p (p^2 - 2p + 1) + (1-p) p^2}{p - p^2}
    = 1
\end{align}

I might discard the \(\sigma_p\) later, but in any case, this is useful for showing the following basic result for my own sanity.

\begin{proposition}
The \(p\)-biased basis functions are orthonormal under \(\Bern(p)^n\).
For any \(S, T \subseteq [n]\), it holds that
\begin{equation*}
    \expval{\alpha \sim \Bern(p)^n}
    \bracks{\chi_S ^p (\alpha) \chi_T ^p (\alpha)}
    = \begin{dcases}
        1, & \text{if \(S = T\)}, \\
        0, & \text{if \(S \neq T\).}
    \end{dcases}
\end{equation*}
\end{proposition}
\begin{proof}
We expand and group the inner product as:
\begin{align*}
    \expval{\alpha \sim \mu_p} \bracks{\chi_S ^p (\alpha) \chi_T ^p (\alpha)}
    &= \expval{\alpha}
    \parens*{\prod_{i \in S} \frac{p - \alpha_i}{\sqrt{p - p^2}}}
    \parens*{\prod_{j \in T} \frac{p - \alpha_j}{\sqrt{p - p^2}}} \\
    &= \expval{\alpha}
    \parens*{\prod_{i \in S \cap T} \parens*{\frac{p - \alpha_i}{\sqrt{p - p^2}}}^2}
    \parens*{\prod_{j \in S \triangle T} \frac{p - \alpha_j}{\sqrt{p - p^2}}} \\
    &= \underbrace{\parens*{\prod_{i \in S \cap T} \expval{\alpha} \parens*{\frac{p - \alpha_i}{\sqrt{p - p^2}}}^2}}_{= 1}
    \underbrace{
    \parens*{\prod_{j \in S \triangle T} \expval{\alpha} \parens*{\frac{p - \alpha_j}{\sqrt{p - p^2}}}}}_{\text{\(= 0\), if \(S \triangle T \neq \emptyset\)}}
    \tag{Independence of \(\alpha_1, \ldots, \alpha_n\)}
\end{align*}
where recall that the symmetric set difference satisfies \(S \triangle T = \emptyset\) iff \(S = T\).
\end{proof}


We are interested in studying how \(M_\lambda\) acts on some \(\chi_S ^p\).
For this, we first have the algebraic relations:
\begin{equation}
    \label{eqn:big_messy}
    M_\lambda \chi_S ^p (\alpha)
    = \expval{z \sim \Bern(\lambda)^n} \chi_S ^p (\alpha \odot z)
    = \expval{\alpha} \prod_{i \in S} \frac{p - \alpha_i z_i}{\sqrt{p - p^2}}
    = \prod_{i \in S} \bracks*{
        \lambda \frac{p - \alpha_i}{\sqrt{p - p^2}} + (1 - \lambda) \frac{p}{\sqrt{p - p^2}}
    }
    = \prod_{i \in S} \frac{p - \lambda \alpha_i}{\sqrt{p - p^2}}
\end{equation}
where we remark the interesting relation: \(M_\lambda \chi_S ^p (\alpha) = \chi_S ^p (\lambda \alpha)\).
There are several ways to analyze this expression.
Two that I think are interesting to look at are (1) with respect to a \(p/\lambda\)-biased basis, and (2) with respect to the original \(p\)-biased basis.

\subsection{Analysis with respect to \((p/\lambda)\)-biased basis}
Continuing from the above derivation, observe that:
\begin{align}
    M_\lambda \chi_S ^p (\alpha)
        &= \prod_{i \in S} \frac{p - \lambda \alpha_i}{\sqrt{p - p^2}} \\
        &= \prod_{i \in S} \lambda \frac{(p / \lambda) - \alpha_i}{\sqrt{p - p^2}} \\
        &= \prod_{i \in S} \lambda \sqrt{\frac{(p/\lambda) - (p/\lambda)^2}{p - p^2}}
        \frac{(p/\lambda) - \alpha_i}{\sqrt{(p/\lambda) - (p/\lambda)^2}}
        \tag{Requires \(p/\lambda \leq 1\)} \\
        &= \prod_{i \in S} \sqrt{\frac{\lambda p - p^2}{p - p^2}} \frac{(p/\lambda) - \alpha_i}{\sqrt{(p/\lambda) - (p/\lambda)^2}} \\
        &= \prod_{i \in S} \sqrt{\frac{\lambda - p}{1 - p}} \frac{(p/\lambda) - \alpha_i}{\sqrt{(p/\lambda) - (p/\lambda)^2}} \\
        &= \parens*{\frac{\lambda - p}{1 - p}}^{\abs{S}/2} \chi_S ^{p/\lambda} (\alpha)
\end{align}
I'd like to emphasize that this change-of-basis interpretation only appears to be valid when \(p \leq \lambda\), because otherwise I fear things might get \(\mbb{C}\)omplicated.
By linearity of \(M_\lambda\), we thus have for any \(h: \{0,1\}^n \to \mbb{R}\) that
\begin{equation}
    M_\lambda h (\alpha)
    = M_\lambda \bracks*{\sum_{S \subseteq [n]} \widehat{h}(S) \chi_S ^p (\alpha)}
    = \sum_{S \subseteq [n]}
        \widehat{M_\lambda h}(S) \chi_S ^{p/\lambda} (\alpha),
    \quad \widehat{M_\lambda h}(S) = \parens*{\frac{\lambda - p}{1 - p}}^{\abs{S}/2} \widehat{h}(S)
\end{equation}
Recalling that a \(p\)-biased basis is orthonormal with respect to the \(p\)-biased hypercube, we thus have the following inequality:
\begin{equation}
    \variance{\alpha \sim p/\lambda} [M_\lambda h (\alpha)]
    \leq \parens*{\frac{\lambda - p}{1 - p}}
    \cdot
    \variance{\alpha' \sim p} [h(\alpha')],
\end{equation}
where we conservatively use the first-order contraction factor.
The relation to stability radii is as follows.
Let \(r < n\) be the radii we are certifying up to, where \(n = d - \norm{\alpha_{\msf{fixed}}}_1\) are the remaining, non-selected features that are still available for including as a perturbation.
We wish to show (perhaps under some nice assumptions), that a smoothed \(M_\lambda h\) achieves better stability at \(R = r/\lambda\) than \(h\) does at \(r\).
We approximate sampling from within these radii by \(\Bern(p/\lambda)\) and \(\Bern(p)\), respectively, such that we have the following \red{relaxation}:
\begin{equation}
    \expval{\alpha \sim p/\lambda} (M_\lambda h(\alpha) - M_\lambda h (0))^2
    \stackrel{?}{\leq} \expval{\alpha' \sim p} (h(\alpha') - h(0))^2
    \tag{Want to show this}
\end{equation}
If we assume without loss of generality that \(h(0) = 0\), and so by extension \(M_\lambda h (0) = 0\) as well due to random masking, the above simplifies to:
\begin{equation}
    \expval{\alpha \sim p / \lambda} M_\lambda h (\alpha)^2
    = \widehat{M_\lambda h}(\emptyset)^2
        + \variance{\alpha \sim p / \lambda} [M_\lambda h (\alpha)]
    \stackrel{?}{\leq}
    \widehat{h}(\emptyset)^2
        + \variance{\alpha' \sim p} [h(\alpha')]
    = \expval{\alpha' \sim p} h(\alpha')^2
\end{equation}
Indeed, this inequality holds because \(\widehat{h}(\emptyset) = \widehat{M_\lambda h}(\emptyset)\) due to non-contraction at \(\emptyset\).


\subsection{Analysis with respect to \(p\)-biased basis}
Let us continue from~\cref{eqn:big_messy}, where we observe that one could have chosen to retain analysis in the \(p\)-basis.
Under this case, a bias term is incurred, such that:
\begin{equation*}
    M_\lambda \chi_S ^p (\alpha)
    = \prod_{i \in S} \bracks*{
        \lambda \frac{p - \alpha_i}{\sqrt{p - p^2}}
        + (1 - \lambda) \frac{p}{\sqrt{p - p^2}}
    }
    = \sum_{T \subseteq S} \lambda^{\abs{T}} \gamma^{\abs{S - T}} \chi_T ^p (\alpha),
    \quad \gamma = (1 - \lambda) \sqrt{\frac{p}{1 - p}},
\end{equation*}
where I will refer to~\cref{lem:mus_chi} for the hopefully more enlightening combinatorial argument.
I am introducing \(\gamma\) because I found it useful for pen-and-paper calculations.
In any case, \(\gamma \leq 1 - \lambda\) only when \(p \leq 1/2\).
With very similar arguments to~\cref{lem:mus_h}, we arrive at:
\begin{equation}
    M_\lambda h (\alpha) = \sum_{T \subseteq [n]} \widehat{M_\lambda h} (T) \chi_T ^p (\alpha),
    \quad \widehat{M_\lambda h} (T) = \lambda^{\abs{T}} \sum_{S \supseteq T} \gamma^{\abs{S - T}} \widehat{h}(S)
\end{equation}
where observe that~\cref{lem:mus_h} is the special case of the unbiased \(p = 1/2\).
The main difficulty in calculating an \(L^2\) in the ``same-basis'' representation is that we inevitably have to handle something of the following form:
\begin{equation}
    \parens*{\widehat{M_\lambda h}(T)}^2
    = \lambda^{2 \abs{T}} \sum_{S, S' \supseteq T} \gamma^{\abs{S - T}} \gamma^{\abs{S' - T}} \widehat{h}(S) \widehat{h}(S'),
\end{equation}
where the cross terms are very annoying.
After consulting ChatGPT, one idea is to suppose that the spectrum is exponentially decaying in the sense that \(\abs{\widehat{h}(S)} \leq \kappa^{\abs{S}}\) for some \(\kappa < 1\).
In this view, we have by (un?)-folding a binomial expansion:
\begin{equation}
    \abs{\widehat{M_\lambda h} (T)}
    \leq \lambda^{\abs{T}} \sum_{S \supseteq T} \gamma^{\abs{S - T}} \kappa ^{\abs{S}}
    = (\lambda\kappa)^{\abs{T}} \sum_{S \supseteq T} (\gamma \kappa)^{\abs{S - T}}
    = (\lambda \kappa)^{\abs{T}} (1 + \gamma \kappa)^{n - \abs{T}}
\end{equation}
Accordingly, we have for the \(L^2\) energy:
\begin{align}
    \sum_{T \subseteq [n]} \abs{\widehat{M_\lambda h} (T)}^2
    \leq \sum_{T \subseteq [n]}
        (\lambda \kappa)^{2\abs{T}} (1 + \gamma \kappa)^{2(n - \abs{T})}
    = \parens*{(\lambda \kappa)^2 + (1 + \gamma \kappa)^2}^n
\end{align}
which compared to the original spectrum's energy is:
\begin{align}
    \sum_{S \subseteq [n]} \abs{\widehat{h}(S)}^2
    \leq \sum_{S \subseteq [n]} \kappa^{2 \abs{S}}
    \leq (1 + \kappa^2)^n
\end{align}
We would thus like to check whether
\begin{align}
    \parens*{(\lambda \kappa)^2 + (1 + \gamma \kappa)^2}^n \stackrel{?}{\leq} (1 + \kappa^2)^n.
\end{align}
Note that the above is an energy comparison; if we want to check for variance, then we note that:
\begin{align*}
    \abs{\widehat{h}(\emptyset)} \leq 1,
    \quad \abs{\widehat{M_\lambda h}(\emptyset} \leq (1 + \gamma \kappa)^n
\end{align*}
I didn't push these through because they didn't feel like it would be very insightful, but you can most likely find nuanced \(\lambda, \gamma, \kappa\) values that make the inequality hold.


==> old/old_smoothing_analysis.tex <==
\section{\red{(OLD) Analysis of Multiplicative Smoothing}}
\label{sec:smoothing_analysis}

We give an analysis of the smoothing operator as described in~\cref{sec:smoothing}.
Recall that this is defined as follows.

\begin{definition}[\citet{xue2024stability}]
For any classifier \(f: \mbb{R}^n \to \mbb{R}^m\) and smoothing parameter \(\lambda \in [0,1]\), define the multiplicative smoothing operator \(M_\lambda\) as:
\begin{equation*}
    M_\lambda f(x) = \expval{z \sim \Bern(\lambda)^n} f(x \odot z),
    \quad \text{where \(z_1, \ldots, z_n \sim \Bern(\lambda)\) are i.i.d. samples.}
\end{equation*}
\end{definition}

Observe that such \(M_\lambda\) is an operator because it maps functions to functions.
For any classifier \(f\) and input \(x \in \mbb{R}^n\), let \(f_x (\alpha) = f(x \odot \alpha)\), where \(\alpha \in \{0,1\}^n\) is the feature attribution that we are evaluating.
Such \(f_x : \{0,1\}^n \to \mbb{R}^m\) is also known as a \textit{Boolean function} because it takes Boolean-valued inputs.
We will analyze the properties of \(f_x\) using techniques from Boolean function analysis~\citep{o2014analysis} and relate them to notions of stability and robustness.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Background on Boolean function analysis}
A key approach in Boolean function analysis is to study functions of the form \(h: \{0,1\}^n \to \mbb{R}\) by their unique \textit{Fourier expansion}:
\begin{equation*}
    h(\alpha) = \sum_{S \subseteq [n]} \widehat{h}(S) \chi_S (\alpha),
    \quad \chi_S(\alpha) 
    = (-1)^{\sum_{i \in S} \alpha_i}
    = \prod_{i \in S} (-1)^{\alpha_i}
    = \prod_{i \in S} (1 - 2\alpha_i),
\end{equation*}
where the summation is indexed by all the \(2^n\) subsets of \([n] = \{1, \ldots, n\}\).
Each subset \(S \subseteq [n]\) is associated with a \textit{Fourier coefficient} (\textit{weight}) \(\widehat{h}(S) \in \mbb{R}\) and \textit{basis function} \(\chi_S : \{0,1\}^n \to \{-1, + 1\}\).
Expressing a Boolean function in this form makes all the \(k = 0, 1, \ldots, n\) degree interactions between input variables into a linear combination, where the degree of \(\widehat{h}(S) \chi_S (\alpha)\) is the size of \(S\).
As an example, consider a function \(\msf{foo} : \{0,1\}^2 \to \mbb{R}\) defined as:
\begin{equation*}
    \msf{foo}(\alpha_1, \alpha_2)
    = 2 + 4 \alpha_1 + 2 \alpha_2 - 16 \alpha_1 \alpha_2
\end{equation*}
which for any \(\alpha \in \{0,1\}^2\) may be rewritten to derive the unique Fourier expansion:
\begin{align} \label{eqn:max2_fourier_expansion}
\begin{split}
    \msf{foo} (\alpha)
    &= 1(-1)^0 + 2 (1 - 2 \alpha_1) + 3 (1 - 2 \alpha_2) - 4 (1 - 2\alpha_1) (1 - 2 \alpha_2) \\
    &= \widehat{\msf{foo}} (\emptyset) \chi_\emptyset (\alpha)
        + \widehat{\msf{foo}} (\{1\})
            \chi_{\{1\}} (\alpha)
        + \widehat{\msf{foo}} (\{2\})
            \chi_{\{2\}} (\alpha)
        + \widehat{\msf{foo}} (\{1,2\})
            \chi_{\{1,2\}} (\alpha),
\end{split}
\end{align}
The basis functions \(\chi_S\) are also known as \textit{parity functions} because they count whether there are an even (\(+1\)) or odd (\(-1\)) number of \(\alpha_i = 1\) for \(i \in S\).
Crucially, they form an orthonormal basis on \(\{0,1\}^n\) via:
\begin{equation*}
    \angles{\chi_S, \chi_T}
    = \frac{1}{2^n} \sum_{\alpha \in \{0,1\}^n} \chi_S (\alpha) \chi_T (\alpha)
    = \begin{dcases}
        1, & S = T \\
        0, & S \neq T
    \end{dcases}
\end{equation*}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Boolean Analytic Results}
A common strategy for studying operators like \(M_\lambda\) is to inspect how they act on each basis function.

\begin{lemma} \label{lem:mus_chi}
For any set \(S \subseteq [n]\) and smoothing parameter \(\lambda \in [0,1]\), the Fourier expansion of \(M_\lambda \chi_S\) is given by:
\begin{equation*}
    M_\lambda \chi_S (\alpha)
    = \sum_{T \subseteq S}
    \lambda^{\abs{T}} (1 - \lambda)^{\abs{S - T}}  \chi_T (\alpha).
\end{equation*}
\end{lemma}
\begin{proof}
We first expand as:
\begin{equation*}
    M_\lambda \chi_S (\alpha)
    = \expval{z \sim \mcal{D}} \chi_S (\alpha \odot z)
    = \expval{z \sim \mcal{D}} \prod_{i \in S} (-1)^{\alpha_i z_i}
    = \prod_{i \in S} \expval{z \sim \mcal{D}} (-1)^{\alpha_i z_i}
    = \prod_{i \in S} \bracks*{(1 - \lambda) + \lambda (-1)^{\alpha_i}},
\end{equation*}
where we used the independence of \(z_1, \ldots, z_n\) to swap the expectation and product.
We then use the distributive property to rewrite the product \(\prod_{i \in S} (\cdots)\) as a summation over \(T \subseteq S\) to get
\begin{equation*}
    M_\lambda \chi_S (\alpha)
    = \sum_{T \subseteq S}
        \parens*{\prod_{j \in S - T} (1 - \lambda)}
        \parens*{\prod_{i \in T} \lambda (-1)^{\alpha_i}}
    = \sum_{T \subseteq S} (1 - \lambda)^{\abs{S - T}} \lambda^{\abs{T}} \chi_T (\alpha),
\end{equation*}
where \(T\) acts like an enumeration over the \(2^n\) different choices of \(z \in \{0,1\}^n\) and recall that \(\chi_T (\alpha) = \prod_{i \in T} (\alpha)\).
\end{proof}

In other words, \(M_\lambda\) redistributes the Fourier weight at each basis \(\chi_S\) over to the \(2^{\abs{S}}\) subsets \(T \subseteq S\) according to a binomial distribution \(\msf{Bin}(\abs{S}, \lambda)\).
Because this redistribution acts linearly on the input, we can visualize \(M_\lambda\) as a \(\mbb{R}^{2^n \times 2^n}\) upper-triangular matrix whose entries are indexed by \(T,S \subseteq [n]\), such that
\begin{equation*}
    (M_\lambda)_{T, S} = \begin{dcases}
        \lambda^{\abs{T}} (1 - \lambda)^{\abs{S - T}}, &T \subseteq S \\
        0, &\text{otherwise}
    \end{dcases}
\end{equation*}
Using the example of \(\msf{foo}\) from~\cref{eqn:max2_fourier_expansion}, the Fourier coefficients of the smoothed \(M_\lambda \msf{foo}\) may be expressed as:
\begin{equation*}
    \begin{bmatrix}
        \widehat{M_\lambda \msf{foo}}(\emptyset) \\
        \widehat{M_\lambda \msf{foo}}(\{1\}) \\
        \widehat{M_\lambda \msf{foo}}(\{2\}) \\
        \widehat{M_\lambda \msf{foo}}(\{1,2\})
    \end{bmatrix}
    = \begin{bmatrix}
        1 & (1 - \lambda) & (1 - \lambda) & (1 - \lambda)^2 \\
        & \lambda & & \lambda (1 - \lambda) \\
        & & \lambda & \lambda (1 - \lambda) \\
        & & & \lambda^2
    \end{bmatrix}
    \begin{bmatrix}
        \widehat{\msf{foo}} (\emptyset) \\
        \widehat{\msf{foo}} (\{1\}) \\
        \widehat{\msf{foo}} (\{2\}) \\
        \widehat{\msf{foo}} (\{1,2\})
    \end{bmatrix}
    = \begin{bmatrix}
        1 + 3\lambda - 4\lambda^2 \\
        -2 \lambda + 4 \lambda^2 \\
        -\lambda + 4 \lambda^2 \\
        - 4\lambda^2
    \end{bmatrix}
\end{equation*}
where recall that
\begin{equation*}
    \widehat{\msf{foo}}(\emptyset) = 1,
    \quad \widehat{\msf{foo}}(\{1\}) = 2,
    \quad \widehat{\msf{foo}}(\{2\}) = 3,
    \quad \widehat{\msf{foo}}(\{1,2\}) = -4.
\end{equation*}
In general, it is helpful to lexicographically sort the rows and columns of \(M_\lambda\) and partition them by degree.
As an example with \(n = 3\), one may write \(M_\lambda \in \mbb{R}^{8 \times 8}\) as:
\begin{equation} \label{eqn:m_matrix_example}
M_\lambda \enskip\cong\quad
\begin{array}{c||c|ccc|ccc|c}
    & \emptyset & \{1\} & \{2\} & \{3\} & \{1,2\} & \{1,3\} & \{2,3\} & \{1,2,3\} \\ \hline \hline
\emptyset & 1 & (1-\lambda) & (1-\lambda) & (1-\lambda) & (1-\lambda)^2 & (1-\lambda)^2 & (1-\lambda)^2 & (1-\lambda)^3 \\ \hline
\{1\}     & & \lambda & & & \lambda(1-\lambda) & \lambda(1-\lambda) & & \lambda(1-\lambda)^2 \\
\{2\}     & & & \lambda & & \lambda(1-\lambda) & & \lambda(1-\lambda) & \lambda(1-\lambda)^2 \\
\{3\}     & & & & \lambda & & \lambda(1-\lambda) & \lambda(1-\lambda) & \lambda(1-\lambda)^2 \\ \hline
\{1,2\}   & & & & & \lambda^2 & & & \lambda^2 (1-\lambda) \\
\{1,3\}   & & & & & & \lambda^2 & & \lambda^2 (1-\lambda) \\
\{2,3\}   & & & & & & & \lambda^2 & \lambda^2 (1-\lambda) \\ \hline
\{1,2,3\} & & & & & & & & \lambda^3 \\
\end{array}
\end{equation}

This visualization will help us reason about later proofs.
Because the columns of \(M_\lambda\) sum to \(1\), we immediately have
\begin{equation*}
    \sum_{T \subseteq [n]} \widehat{M_\lambda h}(T) = \sum_{S \subseteq [n]} \widehat{h}(S),
    \quad \text{for any function \(h: \{0,1\}^n \to \mbb{R}\)}.
\end{equation*}
Moreover, \(M_\lambda h\) is a downshift of \(h\) in the sense that: for each \(T \subseteq [n]\), the Fourier coefficient \(\widehat{M_\lambda h}(T)\) depends only on those of \(\widehat{h}(S)\) for \(S \supseteq T\).
This relation is given as follows.


\begin{lemma} \label{lem:mus_h}
For any function \(h: \{0,1\}^n \to \mbb{R}\) and smoothing parameter \(\lambda \in [0,1]\),
the Fourier expansion of \(M_\lambda h\) is:
\begin{equation*}
    M_\lambda h(\alpha)
    = \sum_{T \subseteq [n]} \widehat{M_\lambda h}(T) \chi_T (\alpha),
    \quad
    \widehat{M_\lambda h}(T)
    = \lambda^{\abs{T}} \sum_{S \supseteq T} (1 - \lambda)^{\abs{S - T}} \widehat{h}(S).
\end{equation*}
\end{lemma}
\begin{proof}
This follows by analyzing the \(T\)-th row of \(M_\lambda\) as in~\cref{eqn:m_matrix_example}.
In particular, we first use~\cref{lem:mus_chi} to derive:
\begin{equation*}
    M_\lambda h(\alpha)
    = \sum_{S \subseteq [n]} \widehat{h}(S) M_\lambda \chi_S (\alpha)
    = \sum_{S \subseteq [n]} \widehat{h}(S) \sum_{T \subseteq S} \lambda^{\abs{T}} (1 - \lambda)^{\abs{S - T}}  \chi_T (\alpha).
\end{equation*}
We next swap the inner and outer summations to write \(M_\lambda h(\alpha) = \sum_{T \subseteq [n]} \chi_T (\alpha) w_T\), where observe that \(w_T\) depends only on \(\widehat{h}(S)\) for \(S \supseteq T\).
Because each such \(\widehat{h}(S)\) is weighted by \(\lambda^{\abs{T}} (1 - \lambda)^{\abs{S - T}}\), we have
\begin{equation*}
    w_T = \sum_{S \supseteq T} \lambda^{\abs{T}} (1 - \lambda)^{\abs{S - T}} \widehat{h} (S).
\end{equation*}
\end{proof}

This expression for \(\widehat{M_\lambda h}(T)\) is useful because it allows us to state a non-trivial contraction result on the spectral mass, i.e., the \(L^1\) norm.
In particular, we give a fine-grained bound on how much mass \(M_\lambda h\) retains for \(\geq k\)-degree terms.

\begin{theorem}[Spectral Mass Contraction]\label{thm:mus_mass_contraction}
For any function \(h: \{0,1\}^n \to \mbb{R}\), smoothing parameter \(\lambda \in [0,1]\), and \(0 \leq k \leq n\), the following inequality holds:
\begin{equation*}
    \sum_{T: \abs{T} \geq k} \abs{\widehat{M_\lambda h}(T)}
    \leq C(k; n, \lambda)
        \sum_{S: \abs{S} \geq k} \abs{\widehat{h}(S)},
\end{equation*}
where \(C(k; n, \lambda)\) is the tail cumulative of \(\msf{Bin}(n, \lambda)\), i.e.,
\(C(k; n, \lambda) = \prob{}[X \geq k]\) for any \(X \sim \msf{Bin}(n, \lambda)\).
\end{theorem}
\begin{proof}
We first apply~\cref{lem:mus_h} to expand each \(\widehat{M_\lambda h}(T)\) and derive
\begin{equation*}
    \sum_{T : \abs{T} \geq k} \abs{\widehat{M_\lambda h}(T)}
    \leq \sum_{T : \abs{T} \geq k} \sum_{S \supseteq T} \lambda^{\abs{T}} (1 - \lambda)^{\abs{S - T}} \abs{\widehat{h}(S)}
    = \sum_{S : \abs{S} \geq k} \abs{\widehat{h}(S)} \underbrace{\sum_{j = k}^{\abs{S}} \binom{\abs{S}}{j} \lambda^{j} (1 - \lambda)^{\abs{S} - j}}_{C(k; \abs{S}, \lambda)}
\end{equation*}
where we re-indexed the summations to track the contribution of each \(\abs{\widehat{h}(S)}\) for \(\abs{S} \geq k\).
As a visual aid, we refer to~\cref{eqn:m_matrix_example}.
Finally, applying \(C(k; \abs{S}, \lambda) \leq C(k; n, \lambda)\) yields the stated contraction factor.
\end{proof}




% Observe that this bound holds with equality if each \(\widehat{h}(S) \geq 0\).





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Relation to Classifier Stability}



==> old/overview_1.tex <==
\input{icml2025/figures/different_kinds_of_stability}

\section{Background and Overview}

First, we will give an overview of feature attributions.
We then discuss the existing studies around hard stability and introduce the notion of soft stability.




\subsection{Feature Attributions as Explanations}

Feature attributions are a popular form of explainability method.
We consider classifiers of the form \(f: \mbb{R}^n \to \mbb{R}^m\), which maps inputs from \(\mbb{R}^{n}\) to logits over \(m\) classes.
Given such a classifier and input \(x \in \mbb{R}^n\), the objective of a feature attribution method is to find a vector \(\alpha \in \mbb{R}^n\), such that \(\alpha_i = 1\) iff the feature \(x_i\) is considered \textit{important} for the prediction \(f(x)\).
The particular notion of importance depends on the choice of attribution method.
For instance, gradient saliency-based methods will take \(\alpha_i \sim \abs{\nabla f(x)_i}\), while Shapley value-based techniques approximate \(\alpha_i\) to be the Shapley value of feature \(x_i\).



While feature attributions are real-valued in general, it is often convenient to consider binary-valued variants.
Indeed, any continuous-valued attribution \(\alpha\) may be binarized with respect to some chosen scheme.
The main benefit of binary-valued feature attributions is that it is simpler to define various properties over them.
Under this scheme, one particular way of evaluating the explainability of a binary-valued attribution \(\alpha \in \{0,1\}^n\) is to see if it can recover the original prediction.
To do this, we first introduce some notation.
Given a classifier \(f: \mbb{R}^{n} \to \mbb{R}^{m}\) and inputs \(x, x' \in \mbb{R}^n\), we write \(f(x) \cong f(x')\) to mean that \(x\) and \(x'\) yield the same class on \(f\), i.e.,
\begin{equation*}
    f(x) \cong f(x')
    \iff
    \argmax_k f(x)_k = \argmax_{k'} f(x')_{k'}.
\end{equation*}
We say that an explanation \(\alpha \in \{0,1\}^n\) is \textit{consistent} for input \(x \in \mbb{R}^{n}\) on classifier \(f\) if \(f(x) \cong f(x \odot \alpha)\), where \(\odot\) is the element-wise product between vectors.
Importantly, while any \(\alpha\) may be proposed as an explanation for an input \(x\) on classifier \(f\), not all explanations are necessarily consistent.



\subsection{Hard Stability and Soft Stability}

\citet{xue2024stability} shows that a number of popular feature attribution methods produce explanations that are sensitive to perturbations in the features.
To mitigate this, they propose a notion of stability as defined below.


\begin{definition}[Hard Stability~\citep{xue2024stability}]\label{def:incremental_stability}
Given a classifier \(f\) and input \(x\), an explanation \(\alpha\) is \textit{stable}~\footnote{
\citet{xue2024stability} actually call this property ``incremental stable'', whereas ``stable'' is defined with a much stricter condition.
}
with radius \(r\) if:
\(f(x \odot \alpha') \cong f(x \odot \alpha)\)
for all \(\alpha' \geq \alpha\) where \(\abs{\alpha' - \alpha} \leq r\).
\end{definition}


% Stability states that no matter how features are added to the attribution, the induced prediction does not change.
% The primary motivation is that the initial explanation \(\alpha\) is sufficiently convincing, such that the unveiling of additional information does not impact the explanatory power of the original \(\alpha\).
% However, stability is hard to certify because there are \(2^{n - \abs{\alpha}}\) different \(\alpha'\) to check.
% To resolve this, the definition of incremental stability is used, which is a local variant of stability.
% As an illustration of both concepts, we refer to the Figure~\red{X}.


This states that adding up to \(r\) new features to \(\alpha\) will not alter the induced prediction.
We refer to this notion as \textit{hard} because it is a \textit{for all} requirement.
Hard stability is actually the standard approach for smoothing-based certificates \red{(CITE)}.
As we will discuss in~\cref{sec:limitations_of_hard_stability}, the main challenge with hard stability is that the guarantees are conservative.
In practice, only a small radius (often \(r \leq 4\)) is certifiable under the hard stability criteria.


This strictness motivates us to present a softer version of stability.
In particular, we are guided by the observation that, in practice, stupid ML practitioners are often satisfied with high-probability guarantees rather than for-all guarantees \red{(CITE)}.
To present soft stability, we first define the set of \(\alpha' \geq \alpha\) with \textit{exactly} \(k\) additive perturbations, as follows:
\begin{equation*}
    \Delta^{(k)}(\alpha)
    \equiv \{\alpha' \in \{0,1\}^n: \alpha' \geq \alpha,\, \abs{\alpha' - \alpha} = k\}
\end{equation*}
When \(\alpha\) is clear from context, we will simply write \(\Delta^{(k)}\) to mean \(\Delta^{(k)}(\alpha)\).
We then use this to present soft stability as follows, in particular through the notion of a \textit{stability rate}.


\begin{definition}[Soft Stability]\label{def:soft_stability}
Given a classifier \(f\) and input \(x\), define the \textit{stability rate} of an explanation \(\alpha\) at radius \(r\) as
\begin{equation*}
    \tau_r (f, x, \alpha) \equiv \min_{k \leq r} \prob{\alpha' \sim \Delta^{(k)}} \bracks*{f(x \odot \alpha') \cong f(x \odot \alpha)}.
\end{equation*}
\end{definition}

We assume that the sampling is uniform over sets unless otherwise specified.
Additionally, we will simply write \(\tau_r\) instead of \(\tau_r (f, x, \alpha)\) when the context is clear.
Observe that for fixed \(f\), \(x\), and \(\alpha\), the value of \(\tau_r\) decreases when \(r\) increases.
This matches intuition because it means that the guarantees one can provide are weaker if the desired radius is larger.


Soft stability may be seen as a relaxation of hard stability.
The semantic interpretation is as that: ``for all \(k \leq r\), a \(k\)-sized perturbation to \(\alpha\) has probability \(\tau_r\) of inducing the same prediction''.
We visualize this in~\cref{fig:hard_stability_vs_soft_stability}.




\paragraph{Alternative Considerations for Stability Rate}
Although we have used a particular definition of stability rate above, alternative definitions are also candidates for consideration.
In particular, one competing definition is to define \(\tau_r\) as ``the probability that some uniformly sampled perturbation of size \(\leq r\)''.
However, this is a weaker (laxer) definition than our chosen definition in~\cref{def:soft_stability}.
We formalize this as follows:
\begin{proposition}
For any classifier \(f\), input \(x\), explanation \(\alpha\), and radius \(r\), we have
\begin{equation*}
    \tau_r (f, x, \alpha) \leq
    \prob{\alpha' \sim \bigcup_{k \leq r} \Delta^{(k)}}
    \bracks*{f(x \odot \alpha') \cong f(x \odot \alpha)}.
\end{equation*}
\end{proposition}
\begin{proof}
We show this in~\cref{prop:our_thing_is_better}.
\end{proof}



==> old/overview_2.tex <==
\section{Background and Overview}

First, we will give an overview of feature attributions.
We then discuss the existing work on hard stability and introduce the notion of soft stability.




\subsection{Feature Attributions as Explanations}

Feature attributions are a popular form of explainability methods.
We consider classifiers of the form \(f: \mbb{R}^n \to \mbb{R}^m\), which maps inputs from \(\mbb{R}^{n}\) to logits over \(m\) classes.
Given such a classifier and input \(x \in \mbb{R}^n\), the objective of a feature attribution method is to find a vector \(\alpha \in \mbb{R}^n\), such that \(\alpha_i\) is large iff the feature \(x_i\) is considered \textit{important} for the prediction \(f(x)\).
\red{(Flesh out)}
The particular notion of importance depends on the choice of attribution method.
For instance, gradient saliency-based methods will take \(\alpha_i \sim \abs{\nabla f(x)_i}\), while Shapley value-based techniques approximate \(\alpha_i\) to be the Shapley value of feature \(x_i\).



While feature attributions are real-valued in general, it is often convenient to consider binary-valued variants.
Indeed, any continuous-valued attribution \(\alpha\) may be binarized with respect to some chosen scheme.
The main benefit of binary-valued feature attributions is that it is simpler to define various properties over them.
Under this scheme, one particular way of evaluating the explainability of a binary-valued attribution \(\alpha \in \{0,1\}^n\) is to see if it can recover the original prediction.
To do this, we first introduce some notation.
For a classifier \(f: \mbb{R}^{n} \to \mbb{R}^{m}\) and inputs \(x, x' \in \mbb{R}^n\), we write \(f(x) \cong f(x')\) to mean that \(x\) and \(x'\) yield the same prediction:
\begin{equation*}
    f(x) \cong f(x')
    \iff
    \argmax_k f(x)_k = \argmax_{k'} f(x')_{k'}.
\end{equation*}

% We say that an explanation \(\alpha \in \{0,1\}^n\) is \textit{consistent} for input \(x \in \mbb{R}^{n}\) on classifier \(f\) if \(f(x) \cong f(x \odot \alpha)\), where \(\odot\) is the element-wise product between vectors.
% Importantly, while any \(\alpha\) may be proposed as an explanation for an input \(x\) on classifier \(f\), not all explanations are necessarily consistent.

For evaluating two explanations \(\alpha, \alpha'\), it is common to compare whether \(f(x \odot \alpha) \cong f(x \odot \alpha')\).
For instance, this is how notions of other perturbation metrics, such as insertion and deletion robustness, may be defined~\citep{nauta2023anecdotal}.


\input{icml2025/figures/different_kinds_of_stability}


\subsection{Hard Stability and Soft Stability}

\citet{xue2024stability} shows that a number of popular feature attribution methods produce explanations that are sensitive to perturbations.
This is formally captured by first an additive perturbation set with respect to a given explanation \(\alpha \in \{0,1\}^n\) as follows:

\begin{definition}[Perturbation Set]
For an explanation \(\alpha\) and radius \(r > 0\), define the \(r\)-perturbation set of \(\alpha\) as:
\begin{equation*}
    \Delta_r (\alpha)
    = \{\alpha' \in \{0,1\}^n: \alpha' \geq \alpha,\, \abs{\alpha' - \alpha} \leq r\}.
\end{equation*}
\end{definition}
When \(\alpha\) is clear from context, we will simply write \(\Delta_r\) to mean \(\Delta_r (\alpha)\).
Intuitively, \(\Delta_r\) corresponds to the set of explanations that are ``more informative'' than \(\alpha\).
If \(\alpha\) were a ``good quality'' explanation, then any \(\alpha' \in \Delta_r\) should satisfy \(f(x \odot \alpha') \cong f(x \odot \alpha)\).
That is, the inclusion of additional information should not change the classifier prediction.
This is the notion that is captured in the definition of hard stability.


\begin{definition}
% [Hard Stability]
[Hard Stability~\citep{xue2024stability}]
\label{def:incremental_stability}
For a classifier \(f\) and input \(x\), the explanation \(\alpha\) is \textit{hard-stable}~\footnote{
\citet{xue2024stability} equivalently call this property ``incrementally stable'' and more broadly define ``stable'' as a stricter property.
}
with radius \(r\) if:
\(f(x \odot \alpha') \cong f(x \odot \alpha)\) for all \(\alpha' \in \Delta_r\).
\end{definition}



This states that adding up to \(r\) new features to \(\alpha\) will not alter the induced prediction.
We refer to this notion as \textit{hard} because it is a \textit{for all} requirement.
Hard stability is actually the standard approach for smoothing-based certificates \red{(CITE)}.
As we will discuss in~\cref{sec:limitations_of_hard_stability}, the main challenge with hard stability is that the guarantees are conservative.
In practice, only a small radius (often \(r \leq 4\)) is certifiable under the hard stability criteria.
This strictness motivates us to present a softer version of stability.


We are motivated by the recent trend of using probabilistic techniques to yield more practically effective guarantees for large black-box models~\citep{angelopoulos2023conformal,ye2024benchmarking}.
We want to find alternatives to hard stability that are more tractable to certify.
Hence, we consider a probabilistic relaxation to hard stability that we call \textit{soft stability}, which is quantified by the notion of a \textit{stability rate} as follows:


\begin{definition}[Soft Stability]\label{def:soft_stability}
For a classifier \(f\) and input \(x\), define the \textit{stability rate} of explanation \(\alpha\) at radius \(r\) as:
\begin{equation*}
    \tau_r (f, x, \alpha) = \prob{\alpha' \sim \Delta_r} \bracks*{f(x \odot \alpha') \cong f(x \odot \alpha)}.
\end{equation*}
\end{definition}

We assume that sampling is uniform over sets unless otherwise specified.
Additionally, we will simply write \(\tau_r\) instead of \(\tau_r (f, x, \alpha)\) when the context is clear.
Soft stability may be seen as a relaxation of hard stability.
The semantic interpretation is that: ``an \(\leq r\)-sized additive perturbation to \(\alpha\) has probability \(\tau_r\) of inducing the same prediction''.
We visualize this in~\cref{fig:hard_stability_vs_soft_stability}.

Observe that for fixed \(f\), \(x\), and \(\alpha\), the value of \(\tau_r\) decreases when \(r\) increases.
This matches intuition because it means that the guarantees one can provide are weaker if the desired radius is larger.







% \paragraph{Alternative Considerations for Stability Rate}
% Although we have used a particular definition of stability rate above, alternative definitions are also candidates for consideration.
% In particular, one competing definition is to define \(\tau_r\) as ``the probability that some uniformly sampled perturbation of size \(\leq r\)''.
% However, this is a weaker (laxer) definition than our chosen definition in~\cref{def:soft_stability}.
% We formalize this as follows:
% \begin{proposition}
% For any classifier \(f\), input \(x\), explanation \(\alpha\), and radius \(r\), we have
% \begin{equation*}
%     \tau_r (f, x, \alpha) \leq
%     \prob{\alpha' \sim \bigcup_{k \leq r} \Delta^{(k)}}
%     \bracks*{f(x \odot \alpha') \cong f(x \odot \alpha)}.
% \end{equation*}
% \end{proposition}
% \begin{proof}
% We show this in~\cref{prop:our_thing_is_better}.
% \end{proof}



==> old/proofs.tex <==
\section{Technical Proofs}

\input{icml2025/sections/appendix_contents/proofs_contents/stability_rate_choices_proof}

\input{icml2025/sections/appendix_contents/proofs_contents/stability_rate_sampling_proof}

==> old/proofs_contents/stability_rate_choices_proof.tex <==

\begin{proposition}\label{prop:our_thing_is_better}
For any classifier \(f\), input \(x\), explanation \(\alpha\), and radius \(r\), we have
\begin{equation*}
    \min_{k \leq r} \prob{\alpha' \sim \Delta^{(k)}} \bracks*{f(x \odot \alpha') \cong f(x \odot \alpha)}
    \leq \prob{\alpha' \sim \bigcup_{k \leq r} \Delta^{(k)}} \bracks*{f (x \odot \alpha') \cong f(x \odot \alpha)}.
\end{equation*}
\end{proposition}
\begin{proof}
First, define
\begin{equation*}
    S^{(k)} = \sum_{\alpha^{(k)} \in \Delta^{(k)}} \mbf{1}\bracks*{f(x \odot \alpha^{(k)}) \cong f(x \odot \alpha)},
\end{equation*}
Because we uniformly sample over sets and there are \(\binom{n}{k}\) elements in each \(\Delta^{(k)} = \{\alpha' : \alpha' \geq \alpha,\,\abs{\alpha'} = k\}\), we have
\begin{align*}
    \min_{k \leq r} \prob{\alpha' \sim \Delta^{(k)}} \bracks*{f(x \odot \alpha') \cong f(x \odot \alpha)}
    &= \min \braces*{
        \frac{S^{(1)}}{\binom{n}{1}},
        \ldots,
        \frac{S^{(r)}}{\binom{n}{r}}
    } \\
    \prob{\alpha' \sim \bigcup_{k \leq r} \Delta^{(k)}} \bracks*{f (x \odot \alpha') \cong f(x \odot \alpha)}
    &= \frac{S^{(1)} + \cdots + S^{(r)}}{\binom{n}{1} + \cdots + \binom{n}{r}}.
\end{align*}
Therefore, it suffices to show that
\begin{equation} \label{eqn:rewritten_with_S}
    \min \braces*{
        \frac{S^{(1)}}{\binom{n}{1}},
        \ldots,
        \frac{S^{(r)}}{\binom{n}{r}}
    }
    \leq \frac{S^{(1)} + \cdots + S^{(r)}}{\binom{n}{1} + \cdots + \binom{n}{r}}.
\end{equation}
To see why this inequality holds, let \(c = \min_k S^{(k)} / \binom{n}{k}\), which implies that \(c \binom{n}{j} \leq S^{(j)}\) for all \(j \leq r\).
Consequently,
\begin{equation*}
    c \bracks*{\binom{n}{1} + \cdots + \binom{n}{r}}
    \leq S^{(1)} + \cdots + S^{(r)},
\end{equation*}
which entails~\cref{eqn:rewritten_with_S}.
\end{proof}


==> old/proofs_contents/stability_rate_sampling_proof.tex <==


\begin{lemma}\label{lem:stability_rate_lemma}
Consider any function \(h: \{0,1\}^p \to \{0,1\}\).
Fix a tolerance \(\varepsilon > 0\), failure probability \(\delta > 0\), and radius \(r > 0\).
Using \(N \geq \log(r/\delta) / (2 \varepsilon^2)\) samples for each \(k = 1, \ldots, r\), let
\begin{equation*}
    \hat{\mu}^{(k)} = \frac{1}{N} \bracks*{ h(\beta_1 ^{(k)}) + \cdots + h(\beta_N ^{(k)})},
    \quad \text{where each \(\beta_i ^{(k)} \sim \{0,1\}^p\) with \(\abs{\beta_i ^{(k)}} = k\), uniformly}.
\end{equation*}
Let \(\hat{\tau} = \min_{k \leq r} \hat{\mu}^{(k)}\) and let \(\tau = \min_{k \leq r} \mu^{(k)}\), where \(\mu^{(k)} = \expval{}[h(\beta^{(k)})]\).
Then, \(\prob{}\bracks*{\tau \geq \hat{\tau} - \varepsilon} \geq 1 - \delta\).
\end{lemma}
\begin{proof}
It suffices to show that
\begin{equation*}
    1 - \prob{}\bracks*{\tau \geq \hat{\tau} - \varepsilon}
    = 1 - \prob{}\bracks*{\bigcap_k \parens*{\mu^{(k)} \geq \hat{\tau} - \varepsilon}}
    = \prob{}\bracks*{\bigcup_k \parens*{\mu^{(k)} < \hat{\tau} - \varepsilon}}
    \leq \delta.
\end{equation*}
This holds by the union bound because for each \(k\):
\begin{align*}
    \prob{}\bracks*{\mu^{(k)} < \hat{\tau} - \varepsilon}
    = \prob{}\bracks*{\mu^{(k)} < \min_j \hat{\mu}^{(j)} - \varepsilon}
    \leq \prob{}\bracks*{\mu^{(k)} < \hat{\mu}^{(k)} - \varepsilon}
    \leq \exp\parens*{-2\varepsilon^2 N}
    \leq \delta / r,
\end{align*}
which follows from Hoeffding's inequality and our choice of \(N\).
\end{proof}


==> old/resnet_stability_vs_lambda_alphas.tex <==
\begin{figure*}[ht]
\centering
\begin{minipage}{0.24\textwidth}
    \centering
    \includegraphics[width=\linewidth]{images/resnet_stability_vs_lambda_alpha0.10.pdf}
\end{minipage}
\hfill
\begin{minipage}{0.24\textwidth}
    \centering
    \includegraphics[width=\linewidth]{images/resnet_stability_vs_lambda_alpha0.15.pdf}
\end{minipage}
\hfill
\begin{minipage}{0.24\textwidth}
    \centering
    \includegraphics[width=\linewidth]{images/resnet_stability_vs_lambda_alpha0.20.pdf}
\end{minipage}
\hfill
\begin{minipage}{0.24\textwidth}
    \centering
    \includegraphics[width=\linewidth]{images/resnet_stability_vs_lambda_alpha0.20.pdf}
\end{minipage}

\caption{The soft stability rates of ResNet18.
}
\label{fig:resnet_stability_vs_lambda_alphas}
\end{figure*}

==> old/roberta_stability_vs_lambda_alphas.tex <==
\begin{figure*}[ht]
\centering
\begin{minipage}{0.24\textwidth}
    \centering
    \includegraphics[width=\linewidth]{images/roberta_stability_vs_lambda_alpha0.10.pdf}
\end{minipage}
\hfill
\begin{minipage}{0.24\textwidth}
    \centering
    \includegraphics[width=\linewidth]{images/roberta_stability_vs_lambda_alpha0.15.pdf}
\end{minipage}
\hfill
\begin{minipage}{0.24\textwidth}
    \centering
    \includegraphics[width=\linewidth]{images/roberta_stability_vs_lambda_alpha0.20.pdf}
\end{minipage}
\hfill
\begin{minipage}{0.24\textwidth}
    \centering
    \includegraphics[width=\linewidth]{images/roberta_stability_vs_lambda_alpha0.20.pdf}
\end{minipage}

\caption{The soft stability rates of RoBERTa.
}
\label{fig:roberta_stability_vs_lambda_alphas}
\end{figure*}

==> old/smoothing_2.tex <==
\section{Mild Smoothing Improves Soft Stability}
\label{sec:smoothing}

Smoothing is commonly used to certify robustness guarantees, such as hard stability~\citep{xue2024stability}, but often at a high cost to the smoothed classifier's accuracy.
Interestingly, however, we found that a milder variant of the smoothing proposed in~\citep{xue2024stability} can improve soft stability while incurring only a minor accuracy trade-off.
We emphasize that the soft stability certification algorithm in~\cref{thm:estimation_algorithm} does \textit{not} require smoothing.
Rather, mildly smoothing the model can empirically improve stability rates.


To formalize this, we now introduce the random masking operator originally used to certify hard stability in~\citet{xue2024stability}, wherein the main idea is for the smoothed classifier to be more robust to the inclusion and exclusion of features.

\begin{definition}
[Random Masking\footnote{
This is also called multiplicative smoothing because the noise scales the input, unlike standard additive noising~\citep{cohen2019certified}.
}]
\label{def:mus_operator}
For any classifier \(f\) and smoothing parameter \(\lambda \in [0,1]\), define the random masking operator \(M_\lambda\) as:
\begin{equation*}
    M_\lambda f (x)
    = \expval{z \sim \Bern (\lambda)^n} f(x \odot z),
    \quad \text{where \(z_1, \ldots, z_n \sim \Bern(\lambda)\) are i.i.d. samples.}
\end{equation*}
\end{definition}

The smoothing parameter \(\lambda\) is the probability that any given feature is kept.
That is, each feature is randomly masked (zeroed, dropped) with probability \(1 - \lambda\).
We say that smoothing becomes stronger as \(\lambda\) shrinks:
at \(\lambda = 1\), no smoothing occurs because \(M_1 f(x) = f(x)\);
at \(\lambda = 1/2\), half the features of \(x \odot z\) are zeroed out on average;
at \(\lambda = 0\), the classifier predicts on an entirely zeroed input because \(M_0 f(x) = f(\mbf{0}_n)\).
In the following, we give an overview of our results in~\cref{sec:main_theory_findings} and a more technical presentation in~\cref{sec:smoothing_analysis_theory}.



\subsection{Summary of Main Theoretical Findings}
\label{sec:main_theory_findings}

Our main theoretical tooling is Boolean function analysis~\citep{o2014analysis}, which studies real-valued functions of Boolean-valued inputs.
To connect this with attribution-masked classification, note that the task of feature selection may be represented with Boolean values.
In other words: for any classifier \(f: \mbb{R}^n \to \mbb{R}^m\) and input \(x \in \mbb{R}^n\), define the function \(f_x (\alpha) = f(x \odot \alpha)\).
Such \(f_x : \{0,1\}^n \to \mbb{R}^m\) is then of the appropriate form for Boolean analytic tooling.
We further observe that \(M_\lambda f(x \odot \alpha) = M_\lambda f_x (\alpha)\), allowing us to study random masking via similar techniques.
This leads to our first result.

\begin{center}
\begin{minipage}{0.95\linewidth}
(\textbf{Result 1})
Smoothed classifiers are more robust to the selection of features.
\end{minipage}
\end{center}

That is, outputs of \(M_\lambda f_x\) across different \(\alpha\) will exhibit less variation compared to those of \(f_x\), which is consistent with the intended behavior of smoothed models.
We offer a nuanced description of this result via \cref{thm:main_body_mus_chi}, \cref{thm:main_body_spectrum_contraction}, and \cref{thm:main_body_variance_reduction}, which characterize and bound various properties of \(M_\lambda\).


While these theorems provide insights into \(M_\lambda\), they do not directly capture the impact of smoothing on stability.
In fact, we found it challenging to establish this connection using standard Boolean analytic techniques, such as those from popular references like~\citet{o2014analysis}.
To overcome this, we introduced a family of non-standard basis functions, using which we arrived at the following result.

\begin{center}
\begin{minipage}{0.95\linewidth}
(\textbf{Result 2})
Smoothing increases a lower bound on the stability rate by a factor of \(\lambda\).
\end{minipage}
\end{center}

Although this result is on the lower bound of stability rates, it aligns with our empirical observation that smoothed classifiers tend to be more stable.
We quantify this improvement as follows: let \(\mcal{Q}\) be a quantity that depends on \(f_x\), then
\begin{equation*}
    1 - \mcal{Q} \leq \tau_r (f_x) \implies 1 - \lambda \mcal{Q} \leq \tau_r (M_\lambda f_x).
\end{equation*}
We describe these non-standard basis functions in~\cref{def:main_body_monotone_basis} and the technical result in~\cref{thm:main_body_monotone_scaling}.


Our theoretical results provide better insight into the empirical behavior of smoothed classifiers.
We provide a novel characterization of random masking, which is qualitatively different from the more commonly studied noising scheme of random flipping~\footnote{
Random flipping, also called the noise operator, is given by \(T_\rho h(\alpha) = \mbb{E}_{z \sim \msf{Bern}(\rho)^n} h((\alpha + z) \,\text{mod}\, 2)\).
}
As a technical contribution, we developed new theoretical tooling as part of our investigation.
In the next section, we discuss the above results in more detail.



\subsection{Technical Results}
\label{sec:smoothing_analysis_theory}

In this section, we give a more technical discussion on random masking.
We defer the extensive details to~\cref{sec:basic_analysis_of_smoothing} and~\cref{sec:stability_via_monotone_basis}, and we refer to ~\cref{sec:boolean_analysis_background} for relevant background on Boolean function analysis.
Our results are primarily given with respect to binary classifiers of the form \(f: \mbb{R}^n \to \mbb{R}\), which is a common simplifying assumption for theoretical analysis~\citep{shalev2014understanding}.


A common approach for studying operators like \(M_\lambda\) is to inspect how they act on a Boolean function's Fourier expansion.
This Fourier expansion uniquely exists for every Boolean function and takes the form:
\begin{equation*}
    f_x (\alpha) = \sum_{S \subseteq [n]} \widehat{f}_x (S) \chi_S (\alpha),
    \quad \text{where} \enskip
    \chi_S (\alpha) = \prod_{i \in S} (-1)^{\alpha_i},
\end{equation*}
where the summation is indexed by all \(2^n\) subsets of \([n] = \{1, \ldots, n\}\).
Each subset \(S \subseteq [n]\) is associated with a Fourier coefficient (weight) \(\widehat{h}(S) \in \mbb{R}\) and basis function \(\chi_S : \{0,1\}^n \to \{\pm 1\}\), which is also known as the standard basis.
For example, the function \(h(\alpha_1, \alpha_2) = \alpha_1 \land \alpha_2\) may be equivalently and uniquely expressed as:
\begin{equation*}
    h(\alpha_1, \alpha_2)
    = \frac{1}{4} \chi_\emptyset (\alpha) + \frac{1}{4} \chi_{\{1\}} (\alpha) + \frac{1}{4} \chi_{\{2\}} (\alpha) + \frac{1}{4} \chi_{\{1,2\}} (\alpha),
\end{equation*}
where \(\alpha = (\alpha_1, \alpha_2)\) and \(\chi_\emptyset (\alpha) = 1\) for all \(\alpha\) by convention.
The effect of \(M_\lambda\) on \(\chi_S\) is as follows.


\begin{theorem}[Spectrum Downshift] \label{thm:main_body_mus_chi}
For any standard basis function \(\chi_S\) and smoothing parameter \(\lambda \in [0,1]\),
\begin{equation*}
    M_\lambda \chi_S (\alpha)
    = \sum_{T \subseteq S}
    \lambda^{\abs{T}} (1 - \lambda)^{\abs{S - T}}  \chi_T (\alpha).
\end{equation*}
\end{theorem}

The effect of this is that spectral weights are shifted from high to low-degree terms according to a binomial distribution of \(\msf{Bin}(\abs{S}, \lambda)\), which shrinks the tail mass of \(M_\lambda f_x\).
This is relevant because Boolean functions with more mass concentrated on low-degree terms tend to be more robust than those with mass concentrated on high-degree terms.
We further quantify this by bounding the remaining spectral mass on the tail.

\begin{theorem}[Tail Mass Contraction]
\label{thm:main_body_spectrum_contraction}
For any function \(h: \{0,1\}^n \to \mbb{R}\), smoothing parameter \(\lambda \in [0,1]\), and \(0 \leq k \leq n\),
\begin{equation*}
    \sum_{T: \abs{T} \geq k} \abs{\widehat{M_\lambda h}(T)}
    \leq C(k, n, \lambda)
        \sum_{S: \abs{S} \geq k} \abs{\widehat{h}(S)},
\end{equation*}
where \(\widehat{h}(S)\) and \(\widehat{M_\lambda h} (S)\) are the weights of \(h\) and \(M_\lambda\) in the standard basis, and \(C(k, n, \lambda) \leq 1\) is the tail cumulative of \(\msf{Bin}(n, \lambda)\), i.e.,
\(C(k, n, \lambda) = \prob{}[X \geq k]\) for any \(X \sim \msf{Bin}(n, \lambda)\).
\end{theorem}

This result gives a bound on how much the spectral mass contracts past a certain degree.
Because \(C(k, n, \lambda) \leq C(k, n, \lambda')\) for all \(\lambda \leq \lambda'\), this suggests that stronger smoothing causes the tail mass to shrink faster.
While spectral tail mass contraction is a good qualitative description of how the operator \(M_\lambda\) changes a function, it does not directly describe sensitivity.
Under some technical conditions, we can do so.


\begin{theorem}[Variance Reduction]
\label{thm:main_body_variance_reduction}
For any function \(h: \{0,1\}^n \to \mbb{R}\) and smoothing parameter \(\lambda \in [p,1]\),
\begin{equation*}
    \variance{\alpha \sim \Bern(p/\lambda)^n} \bracks*{M_\lambda h(\alpha)}
    \leq \parens*{\frac{\lambda - p}{1 - p}} \variance{\alpha \sim \Bern(p)^n} \bracks*{h (\alpha)}.
\end{equation*}
If the function is centered at \(h(\mbf{0}_n) = 0\), then we also have:
\begin{equation*}
    \expval{\alpha \sim \Bern(p/\lambda)^n} \bracks*{M_\lambda h(\alpha) ^2}
    \leq \expval{\alpha \sim \Bern(p)} \bracks*{h(\alpha)^2}.
\end{equation*}
\end{theorem}

This result shows that \(M_\lambda f_x\) remains less sensitive than \(f_x\) even when more features are selected for its input on average, as \(p/\lambda \geq p\).
While a variance reduction better captures improved robustness, we emphasize that both \(\msf{Bern}(p/\lambda)^n\) and \(\msf{Bern}(p)\) are only superficially similar to \(\Delta_r (\alpha)\) if one takes \(p = r / (n - \norm{\alpha}_0)\).
Thus, there is still a gap in directly establishing a result for stability.
To overcome this gap, our main technical innovation is to introduce a set of non-standard basis functions as follows.


\begin{definition}[Monotone Basis]
\label{def:main_body_monotone_basis}
For any subset \(S \subseteq [n]\), define its respective monotone basis function as:
\begin{equation*}
    \mbf{1}_S (\alpha) = \begin{dcases}
        1, & \text{if \(\alpha_i = 1\) for all \(i \in S\)}, \\
        0, & \text{otherwise}.
    \end{dcases}
\end{equation*}
\end{definition}

The monotone basis provides a direct encoding of set inclusion.
For example, the earlier instance of \(h(\alpha_1, \alpha_2) = \alpha_1 \land \alpha_2\) is now concisely represented as \(h(\alpha) = \mbf{1}_{\{1,2\}} (\alpha)\).
As with the standard basis \(\chi_S\), the monotone basis also admits a unique expansion for any Boolean function \(f_x\):
\begin{equation*}
    f_x (\alpha) = \sum_{T \subseteq [n]} \widetilde{f}_x (T) \mbf{1}_T (\alpha),
    \quad \widetilde{f}_x (T) = f_x (T) - \sum_{S \subsetneq T} \widetilde{f}_x (S)
\end{equation*}
where let \(\widetilde{f}_x (S)\) denote the monotone coefficient of \(S\).
Crucially, the monotone basis exhibits the properties that let us establish direct lower bounds on the stability rate of the smoothed classifier.
Under a further simplifying assumption that \(f_x (\alpha') \cong f(\alpha)\) when \(\abs{f_x(\alpha') - f_x(\alpha)} \leq 1/2\), we arrive at the following result.


\begin{theorem}[Smoothed Stability]
\label{thm:main_body_monotone_scaling}
The stability rate of a binary classifier \(h: \{0,1\}^n \to [0,1]\) is bounded by
\begin{equation*}
    1 - \tau_r (h) \leq \mcal{Q}\parens*{\braces{\widetilde{h}(S) : \abs{S} \leq r}},
\end{equation*}
where \(\mcal{Q}\) depends on the monotone weights of degree \(\leq r\).
For any \(\lambda \in [0,1]\), we also have:
\begin{equation*}
    1 - \tau_r (M_\lambda h) \leq \lambda \mcal{Q}\parens*{\braces{\widetilde{h}(S) : \abs{S} \leq r}}.
\end{equation*}
\end{theorem}

This result quantifies the improvement in soft stability due to smoothing, wherein the worst-case bound shrinks by a factor of \(\lambda\).
We present extensive details in~\cref{sec:stability_via_monotone_basis}.




==> old/smoothing_analysis_1.tex <==
\section{\red{(OLD) Analysis of Multiplicative Smoothing}}
\label{sec:smoothing_analysis}

We give an analysis of the smoothing operator as described in~\cref{sec:smoothing}.
Recall that this is defined as follows.

\begin{definition}[\citet{xue2024stability}]
For any classifier \(f: \mbb{R}^n \to \mbb{R}^m\) and smoothing parameter \(\lambda \in [0,1]\), define the multiplicative smoothing operator \(M_\lambda\) as:
\begin{equation*}
    M_\lambda f(x) = \expval{z \sim \msf{Bern}(\lambda)^n} f(x \odot z),
    \quad \text{where \(z_1, \ldots, z_n \sim \msf{Bern}(\lambda)\) are i.i.d. samples.}
\end{equation*}
\end{definition}

Observe that such \(M_\lambda\) is an operator because it maps functions to functions.
For any classifier \(f\) and input \(x \in \mbb{R}^n\), let \(f_x (\alpha) = f(x \odot \alpha)\), where \(\alpha \in \{0,1\}^n\) is the feature attribution that we are evaluating.
Such \(f_x : \{0,1\}^n \to \mbb{R}^m\) is also known as a \textit{Boolean function} because it takes Boolean-valued inputs.
We will analyze the properties of \(f_x\) using techniques from Boolean analysis~\citep{o2014analysis} and relate them to notions of stability and robustness.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Background on Boolean Analysis}
A key approach in Boolean analysis is to study functions of form \(h: \{0,1\}^n \to \mbb{R}\) by their unique \textit{Fourier expansion}:
\begin{equation*}
    h(\alpha) = \sum_{S \subseteq [n]} \widehat{h}(S) \chi_S (\alpha),
    \quad \chi_S(\alpha) 
    = (-1)^{\sum_{i \in S} \alpha_i}
    = \prod_{i \in S} (-1)^{\alpha_i}
    = \prod_{i \in S} (1 - 2\alpha_i),
\end{equation*}
where the summation is indexed by all the \(2^n\) subsets of \([n] = \{1, \ldots, n\}\).
Each subset \(S \subseteq [n]\) is associated with a \textit{Fourier coefficient} (\textit{weight}) \(\widehat{h}(S) \in \mbb{R}\) and \textit{basis function} \(\chi_S : \{0,1\}^n \to \{-1, + 1\}\).
Expressing a Boolean function in this form makes all the \(k = 0, 1, \ldots, n\) degree interactions between input variables into a linear combination, where the degree of \(\widehat{h}(S) \chi_S (\alpha)\) is the size of \(S\).
As an example, consider a function \(\msf{foo} : \{0,1\}^2 \to \mbb{R}\) defined as:
\begin{equation*}
    \msf{foo}(\alpha_1, \alpha_2)
    = 2 + 4 \alpha_1 + 2 \alpha_2 - 16 \alpha_1 \alpha_2
\end{equation*}
which for any \(\alpha \in \{0,1\}^2\) may be rewritten to derive the unique Fourier expansion:
\begin{align} \label{eqn:max2_fourier_expansion}
\begin{split}
    \msf{foo} (\alpha)
    &= 1(-1)^0 + 2 (1 - 2 \alpha_1) + 3 (1 - 2 \alpha_2) - 4 (1 - 2\alpha_1) (1 - 2 \alpha_2) \\
    &= \widehat{\msf{foo}} (\emptyset) \chi_\emptyset (\alpha)
        + \widehat{\msf{foo}} (\{1\})
            \chi_{\{1\}} (\alpha)
        + \widehat{\msf{foo}} (\{2\})
            \chi_{\{2\}} (\alpha)
        + \widehat{\msf{foo}} (\{1,2\})
            \chi_{\{1,2\}} (\alpha),
\end{split}
\end{align}
The basis functions \(\chi_S\) are also known as \textit{parity functions} because they count whether there are an even (\(+1\)) or odd (\(-1\)) number of \(\alpha_i = 1\) for \(i \in S\).
Crucially, they form an orthonormal basis on \(\{0,1\}^n\) via:
\begin{equation*}
    \angles{\chi_S, \chi_T}
    = \frac{1}{2^n} \sum_{\alpha \in \{0,1\}^n} \chi_S (\alpha) \chi_T (\alpha)
    = \begin{dcases}
        1, & S = T \\
        0, & S \neq T
    \end{dcases}
\end{equation*}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Boolean Analytic Results}
A common strategy for studying operators like \(M_\lambda\) is to inspect how they act on each basis function.

\begin{lemma} \label{lem:mus_chi}
For any set \(S \subseteq [n]\) and smoothing parameter \(\lambda \in [0,1]\), the Fourier expansion of \(M_\lambda \chi_S\) is given by:
\begin{equation*}
    M_\lambda \chi_S (\alpha)
    = \sum_{T \subseteq S}
    \lambda^{\abs{T}} (1 - \lambda)^{\abs{S - T}}  \chi_T (\alpha).
\end{equation*}
\end{lemma}
\begin{proof}
We first expand as:
\begin{equation*}
    M_\lambda \chi_S (\alpha)
    = \expval{z \sim \mcal{D}} \chi_S (\alpha \odot z)
    = \expval{z \sim \mcal{D}} \prod_{i \in S} (-1)^{\alpha_i z_i}
    = \prod_{i \in S} \expval{z \sim \mcal{D}} (-1)^{\alpha_i z_i}
    = \prod_{i \in S} \bracks*{(1 - \lambda) + \lambda (-1)^{\alpha_i}},
\end{equation*}
where we used the independence of \(z_1, \ldots, z_n\) to swap the expectation and product.
We then use the distributive property to rewrite the product \(\prod_{i \in S} (\cdots)\) as a summation over \(T \subseteq S\) to get
\begin{equation*}
    M_\lambda \chi_S (\alpha)
    = \sum_{T \subseteq S}
        \parens*{\prod_{j \in S - T} (1 - \lambda)}
        \parens*{\prod_{i \in T} \lambda (-1)^{\alpha_i}}
    = \sum_{T \subseteq S} (1 - \lambda)^{\abs{S - T}} \lambda^{\abs{T}} \chi_T (\alpha),
\end{equation*}
where \(T\) acts like an enumeration over the \(2^n\) different choices of \(z \in \{0,1\}^n\) and recall that \(\chi_T (\alpha) = \prod_{i \in T} (\alpha)\).
\end{proof}

In other words, \(M_\lambda\) redistributes the Fourier weight at each basis \(\chi_S\) over to the \(2^{\abs{S}}\) subsets \(T \subseteq S\) according to a binomial distribution \(\msf{Bin}(\abs{S}, \lambda)\).
Because this redistribution acts linearly on the input, we can visualize \(M_\lambda\) as a \(\mbb{R}^{2^n \times 2^n}\) upper-triangular matrix whose entries are indexed by \(T,S \subseteq [n]\), such that
\begin{equation*}
    (M_\lambda)_{T, S} = \begin{dcases}
        \lambda^{\abs{T}} (1 - \lambda)^{\abs{S - T}}, &T \subseteq S \\
        0, &\text{otherwise}
    \end{dcases}
\end{equation*}
Using the example of \(\msf{foo}\) from~\cref{eqn:max2_fourier_expansion}, the Fourier coefficients of the smoothed \(M_\lambda \msf{foo}\) may be expressed as:
\begin{equation*}
    \begin{bmatrix}
        \widehat{M_\lambda \msf{foo}}(\emptyset) \\
        \widehat{M_\lambda \msf{foo}}(\{1\}) \\
        \widehat{M_\lambda \msf{foo}}(\{2\}) \\
        \widehat{M_\lambda \msf{foo}}(\{1,2\})
    \end{bmatrix}
    = \begin{bmatrix}
        1 & (1 - \lambda) & (1 - \lambda) & (1 - \lambda)^2 \\
        & \lambda & & \lambda (1 - \lambda) \\
        & & \lambda & \lambda (1 - \lambda) \\
        & & & \lambda^2
    \end{bmatrix}
    \begin{bmatrix}
        \widehat{\msf{foo}} (\emptyset) \\
        \widehat{\msf{foo}} (\{1\}) \\
        \widehat{\msf{foo}} (\{2\}) \\
        \widehat{\msf{foo}} (\{1,2\})
    \end{bmatrix}
    = \begin{bmatrix}
        1 + 3\lambda - 4\lambda^2 \\
        -2 \lambda + 4 \lambda^2 \\
        -\lambda + 4 \lambda^2 \\
        - 4\lambda^2
    \end{bmatrix}
\end{equation*}
where recall that
\begin{equation*}
    \widehat{\msf{foo}}(\emptyset) = 1,
    \quad \widehat{\msf{foo}}(\{1\}) = 2,
    \quad \widehat{\msf{foo}}(\{2\}) = 3,
    \quad \widehat{\msf{foo}}(\{1,2\}) = -4.
\end{equation*}
In general, it is helpful to lexicographically sort the rows and columns of \(M_\lambda\) and partition them by degree.
As an example with \(n = 3\), one may write \(M_\lambda \in \mbb{R}^{8 \times 8}\) as:
\begin{equation} \label{eqn:m_matrix_example}
M_\lambda \enskip\cong\quad
\begin{array}{c||c|ccc|ccc|c}
    & \emptyset & \{1\} & \{2\} & \{3\} & \{1,2\} & \{1,3\} & \{2,3\} & \{1,2,3\} \\ \hline \hline
\emptyset & 1 & (1-\lambda) & (1-\lambda) & (1-\lambda) & (1-\lambda)^2 & (1-\lambda)^2 & (1-\lambda)^2 & (1-\lambda)^3 \\ \hline
\{1\}     & & \lambda & & & \lambda(1-\lambda) & \lambda(1-\lambda) & & \lambda(1-\lambda)^2 \\
\{2\}     & & & \lambda & & \lambda(1-\lambda) & & \lambda(1-\lambda) & \lambda(1-\lambda)^2 \\
\{3\}     & & & & \lambda & & \lambda(1-\lambda) & \lambda(1-\lambda) & \lambda(1-\lambda)^2 \\ \hline
\{1,2\}   & & & & & \lambda^2 & & & \lambda^2 (1-\lambda) \\
\{1,3\}   & & & & & & \lambda^2 & & \lambda^2 (1-\lambda) \\
\{2,3\}   & & & & & & & \lambda^2 & \lambda^2 (1-\lambda) \\ \hline
\{1,2,3\} & & & & & & & & \lambda^3 \\
\end{array}
\end{equation}

This visualization will help us reason about later proofs.
Because the columns of \(M_\lambda\) sum to \(1\), we immediately have
\begin{equation*}
    \sum_{T \subseteq [n]} \widehat{M_\lambda h}(T) = \sum_{S \subseteq [n]} \widehat{h}(S),
    \quad \text{for any function \(h: \{0,1\}^n \to \mbb{R}\)}.
\end{equation*}
Moreover, \(M_\lambda h\) is a downshift of \(h\) in the sense that: for each \(T \subseteq [n]\), the Fourier coefficient \(\widehat{M_\lambda h}(T)\) depends only on those of \(\widehat{h}(S)\) for \(S \supseteq T\).
This relation is given as follows.


\begin{lemma} \label{lem:mus_h}
For any function \(h: \{0,1\}^n \to \mbb{R}\) and smoothing parameter \(\lambda \in [0,1]\),
the Fourier expansion of \(M_\lambda h\) is:
\begin{equation*}
    M_\lambda h(\alpha)
    = \sum_{T \subseteq [n]} \widehat{M_\lambda h}(T) \chi_T (\alpha),
    \quad
    \widehat{M_\lambda h}(T)
    = \lambda^{\abs{T}} \sum_{S \supseteq T} (1 - \lambda)^{\abs{S - T}} \widehat{h}(S).
\end{equation*}
\end{lemma}
\begin{proof}
This follows by analyzing the \(T\)-th row of \(M_\lambda\) as in~\cref{eqn:m_matrix_example}.
In particular, we first use~\cref{lem:mus_chi} to derive:
\begin{equation*}
    M_\lambda h(\alpha)
    = \sum_{S \subseteq [n]} \widehat{h}(S) M_\lambda \chi_S (\alpha)
    = \sum_{S \subseteq [n]} \widehat{h}(S) \sum_{T \subseteq S} \lambda^{\abs{T}} (1 - \lambda)^{\abs{S - T}}  \chi_T (\alpha).
\end{equation*}
We next swap the inner and outer summations to write \(M_\lambda h(\alpha) = \sum_{T \subseteq [n]} \chi_T (\alpha) w_T\), where observe that \(w_T\) depends only on \(\widehat{h}(S)\) for \(S \supseteq T\).
Because each such \(\widehat{h}(S)\) is weighted by \(\lambda^{\abs{T}} (1 - \lambda)^{\abs{S - T}}\), we have
\begin{equation*}
    w_T = \sum_{S \supseteq T} \lambda^{\abs{T}} (1 - \lambda)^{\abs{S - T}} \widehat{h} (S).
\end{equation*}
\end{proof}

This expression for \(\widehat{M_\lambda h}(T)\) is useful because it allows us to state a non-trivial contraction result on the spectral mass, i.e., the \(L^1\) norm.
In particular, we give a fine-grained bound on how much mass \(M_\lambda h\) retains for \(\geq k\)-degree terms.

\begin{theorem}[Spectral Mass Contraction]\label{thm:mus_mass_contraction}
For any function \(h: \{0,1\}^n \to \mbb{R}\), smoothing parameter \(\lambda \in [0,1]\), and \(0 \leq k \leq n\), the following inequality holds:
\begin{equation*}
    \sum_{T: \abs{T} \geq k} \abs{\widehat{M_\lambda h}(T)}
    \leq C(k; n, \lambda)
        \sum_{S: \abs{S} \geq k} \abs{\widehat{h}(S)},
\end{equation*}
where \(C(k; n, \lambda)\) is the tail cumulative of \(\msf{Bin}(n, \lambda)\), i.e.,
\(C(k; n, \lambda) = \prob{}[X \geq k]\) for any \(X \sim \msf{Bin}(n, \lambda)\).
\end{theorem}
\begin{proof}
We first apply~\cref{lem:mus_h} to expand each \(\widehat{M_\lambda h}(T)\) and derive
\begin{equation*}
    \sum_{T : \abs{T} \geq k} \abs{\widehat{M_\lambda h}(T)}
    \leq \sum_{T : \abs{T} \geq k} \sum_{S \supseteq T} \lambda^{\abs{T}} (1 - \lambda)^{\abs{S - T}} \abs{\widehat{h}(S)}
    = \sum_{S : \abs{S} \geq k} \abs{\widehat{h}(S)} \underbrace{\sum_{j = k}^{\abs{S}} \binom{\abs{S}}{j} \lambda^{j} (1 - \lambda)^{\abs{S} - j}}_{C(k; \abs{S}, \lambda)}
\end{equation*}
where we re-indexed the summations to track the contribution of each \(\abs{\widehat{h}(S)}\) for \(\abs{S} \geq k\).
As a visual aid, we refer to~\cref{eqn:m_matrix_example}.
Finally, applying \(C(k; \abs{S}, \lambda) \leq C(k; n, \lambda)\) yields the stated contraction factor.
\end{proof}

% Observe that this bound holds with equality if each \(\widehat{h}(S) \geq 0\).





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Relation to Classifier Stability}



==> old/smoothing_analysis_3.tex <==
\section{Mild Smoothing Improves Stability}
\label{sec:smoothing}

Although soft stability is applicable to both smoothed and unsmoothed models, it turns out that mildly smoothing the model can greatly improve the soft stability rate.
We emphasize that to certify soft stability rates, one does not need a smoothed model.
Rather, a smoothed model helps attain better soft stability rates.


In particular, we show that multiplicative smoothing~\citet{xue2024stability}, which was originally designed to certify hard stability radii, is also applicable to improving soft stability guarantees.
The main idea is to randomly drop (i.e., zero-out) features in \(x\) before passing it to \(f\).

\begin{definition}
% [Multiplicative Smoothing]
[\citet{xue2024stability}]
% [Multiplicative Smoothing~\citep{xue2024stability}]
\label{def:mus_operator}
For any classifier \(f\) and smoothing parameter \(\lambda \in [0,1]\), define the multiplicative smoothing operator \(M_\lambda\) as:
\begin{equation*}
    M_\lambda f (x)
    = \expval{z \sim \msf{Bern} (\lambda)^n} f(x \odot z),
\end{equation*}
where \(z_1, \ldots, z_n \sim \msf{Bern}(\lambda)\) are i.i.d. samples.
\end{definition}

The smoothed classifier is \(\tilde{f} = M_\lambda f\).
This procedure is so called because the noise multiplies the input, which is in contrast to more classic smoothing methods that directly add noise to the input~\citep{cohen2019certified}.
One can interpret \(\lambda\) as the probability that each feature is kept.
At a boundary case of \(\lambda = 0\), we have the evaluation of \(f\) on the all-zeros input with \(M_0 f(x) = f(\mbf{0}_n)\).
On the other hand, taking \(\lambda = 1\) yields the identity transformer via \(M_1 f(x) = f(x)\).


\subsection{Differences between Soft vs. Hard Stability}

The application of multiplicative smoothing to the soft stability case.
For hard stability, one needs \(\lambda \leq 1/2\) to yield non-trivial guarantees because of the way Lipschitz constants are calculated.
In such cases, the smoothed classifier often suffers a large accuracy loss because, on average, at least half of the input is zeroed out.
This is not true for soft stability, wherein values as \(\lambda \approx 1\) empirically suffice to yield considerable improvements.


Moreover, the theoretical objectives of smoothing are different in the hard and soft settings.
In the hard setting, the objective is to establish a Lipschitz constant for the smoothed classifier that may be used to do a conservative upper bound on the certifiable radius.
The soft stability certificate, however, depends purely on sampling and does not require the Lipschitz constant.
Instead, the main objective of smoothing can be understood in terms of manipulations of the classifier's Fourier spectrum, as we explain next.


% \paragraph{Probabilistic vs. Deterministic Smoothing}
% One advantage of the 



% \paragraph{Multiplicative Smoothing Improves Stability Rate}


% We later show in \red{(SECTION)} that the smoothed classifier \(M_\lambda f\) can easily attain better stability rates than \(f\) with only minor trade-offs in classification accuracy and evaluation cost.
% Below, we discuss some important theoretical properties of \(M_\lambda\).


% \red{Although we use multiplicative smoothing as in Xue, here are some remarkable things about our particular application compared to theirs}






\subsection{Theoretical Analysis}

We empirically observe that \(M_\lambda f\) attains better stability rates than \(f\), even for \(\lambda \approx 1\).
To explain this behavior, we do a theoretical analysis of multiplicative smoothing as defined in~\cref{def:mus_operator} using tooling from Boolean analysis~\citep{o2014analysis}, where our main result is informally stated as follows.

In Boolean analysis, it is common to view functions by decomposing them into a linear combination of basis functions.

\begin{equation*}
    h(\alpha) = \sum_{S \subseteq [n]} \widehat{h}(S) \varphi_S (\alpha)
\end{equation*}

where \(\widehat{h}(S)\) are the weights and \(\varphi_S : \{0,1\}^n \to \mbb{R}\) is a basis function.


We consider different choices for \(S\).

\begin{definition}[\(p\)-Biased Basis]
For any subset \(S \subseteq [n]\), define its corresponding \(p\)-biased Fourier basis function as:
\begin{equation*}
    \chi_S ^p (\alpha) = \prod_{i \in S} \frac{p - \alpha_i}{\sqrt{p - p^2}}.
\end{equation*}
\end{definition}



\begin{lemma}[Spectrum Shift]
For any \(p\)-biased basis function \(\chi_S ^p\) and smoothing parameter \(\lambda \in [p, 1]\),
\begin{equation*}
    M_\lambda \chi_S ^p (\alpha) = \parens*{\frac{\lambda - p}{1 - p}}^{\abs{S / 2}} \chi_S ^{p/\lambda} (\alpha)
\end{equation*}
\end{lemma}


\begin{lemma}[Variance Reduction]
For any function \(h: \{0,1\}^n \to \mbb{R}\) and smoothing parameter \(\lambda \in [p,1]\),
\begin{equation*}
    \variance{\alpha \sim \msf{Bern}(p/\lambda)^n} \bracks*{M_\lambda h(\alpha)}
    \leq \parens*{\frac{\lambda - p}{1 - p}} \variance{\alpha \sim \msf{Bern}(p)^n} \bracks*{h (\alpha)}.
\end{equation*}
\end{lemma}


The monotone basis function is defined as

\begin{definition}[Monotone Basis]
For any subset \(S \subseteq [n]\), define its corresponding monotone basis function as:
\begin{equation*}
    \mbf{1}_S (\alpha) = \begin{dcases}
        1, & \text{\(\alpha_i = 1\) for all \(i \in S\)}, \\
        0, & \text{otherwise}.
    \end{dcases}
\end{equation*}

\end{definition}

% \begin{proposition}[Informal]
% Smoothing decreases the variance when measured in the right basis.
% \end{proposition}


The main idea is to measure how \(M_\lambda f(x \odot \alpha)\) varies as \(\alpha\) is additively perturbed.

We make several simplifying assumptions to make the analysis tractable.
We later show that these assumptions are well-supported by numerical experiments.


First, we reparametrize this in terms of the perturbation.
Let \(\alpha' = \alpha \oplus \delta\), where \(\delta \in \{0,1\}^{d}\) with \(d = n - \norm{\alpha}_0\) is the set of perturbations and we implicily define \(\oplus\) to act as addition on the appropriate coordinates.

This lets us write \(g(\delta) = f(x \odot (\alpha \oplus \delta))\).

Observe that we then have \(g(0) = f(x \odot \alpha)\).

At this point, the stability rate is now defined as

\begin{equation*}
% \label{eqn:stability_g_delta}
    \prob{\delta \sim \Delta_r (\mbf{0}_d)}
    \bracks{g(\delta) \cong g(\mbf{0}_d)}
\end{equation*}


Second, we relax the \(\cong\) condition to one involving norms.
Intuitively, the above stability is high only when the following expression is small:
\begin{equation*}
    \expval{\delta \sim \Delta_r (\mbf{0}_d)}
    \bracks*{\norm{g(\delta) - g(\mbf{0}_d)}_2 ^2}
\end{equation*}


We make two additional simplifications to the analysis.
First, we suppose that the classifier is scalar-valued and zero-centered, such that it becomes equivalent to considering a binary classification task, wherein a threshold on the value decides whether the input is ``class A'' or ``class B''.
In this case, we have
\begin{equation*}
    % \expval{\delta \sim \Delta_r (\mbf{0}_d)}
    % \bracks*{\norm{g(\delta) - g(\mbf{0}_d)}_2 ^2}
    % =
    % \expval{\delta \sim \Delta_r (\mbf{0}_d)} \bracks*{g(\delta)^2 - 2 g(\delta) g(\mbf{0}_d) + g(\mbf{0}_d)^2}
    \expval{\delta \sim \Delta_r (\mbf{0}_d)} \bracks*{g(\delta)^2}
\end{equation*}



We further approximate \(\Delta_r (\mbf{0}_d)\) using \(\msf{Bern}(p)^d\), where \(p = r/d\).
Because the mass in \(\Delta_r (\mbf{0}_d)\) is concentrated at things \(r\)-distance away, using a Bernoulli to approximate this shares a similar mass distribution.
We have now arrived at the following setup

\begin{equation*}
    \expval{\delta \sim \msf{Bern}(p)^d} \bracks*{g(\delta)^2}
\end{equation*}


\begin{theorem}

\begin{equation*}
    \expval{\delta \sim \msf{Bern}(p/\lambda)^d} \bracks*{(M_\lambda g(\delta))^2}
    \leq \expval{\delta \sim \msf{Bern}(p)^d} \bracks*{g(\delta)^2}.
\end{equation*}
\end{theorem}


\begin{theorem}
\begin{equation*}
    \variance{\delta \sim \msf{Bern}(p/\lambda)^d} \bracks*{M_\lambda g(\delta)}
    \leq \parens*{\frac{\lambda - p}{1 - p}} \variance{\delta \sim \msf{Bern}(p)^d} \bracks*{g(\delta)}
\end{equation*}
\end{theorem}


% \input{figures/smoothing_frequency_shift_example}




==> old/smoothing_analysis_4.tex <==
\section{Analysis of Smoothing with Standard Techniques}
\label{sec:basic_analysis_of_smoothing}


In this section, we analyze the random masking operator using standard tooling from Boolean function analysis.
Recall that this operator is defined as follows.


\begin{definition}[\citet{xue2024stability}]
For any classifier \(f: \mbb{R}^n \to \mbb{R}^m\) and smoothing parameter \(\lambda \in [0,1]\), define the random masking operator \(M_\lambda\) as:
\begin{equation*}
    M_\lambda f(x) = \expval{z \sim \Bern(\lambda)^n} f(x \odot z),
    \quad \text{where \(z_1, \ldots, z_n \sim \Bern(\lambda)\) are i.i.d. samples.}
\end{equation*}
\end{definition}

Tooling from Boolean analysis is applicable to \(M_\lambda\) in the following manner.
For any function \(f: \mbb{R}^n \to \mbb{R}^m\) and input \(x \in \mbb{R}^n\), define the function \(f_x (\alpha) = f(x \odot \alpha)\).
Such \(f_x: \{0,1\}^n \to \mbb{R}^m\) is then a Boolean function, which then satisfies the following relation:
\begin{equation*}
    M_\lambda f(x \odot \alpha)
    = M_\lambda f_x (\alpha)
    = M_\lambda f_{x \odot \alpha} (\mbf{1}_n).
\end{equation*}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Background on Boolean function analysis}
\label{sec:boolean_analysis_background}
A key approach in Boolean function analysis is to study functions of the form \(h: \{0,1\}^n \to \mbb{R}\) by their unique \textit{Fourier expansion}:
\begin{equation*}
    h(\alpha) = \sum_{S \subseteq [n]} \widehat{h}(S) \chi_S (\alpha),
    \quad \text{where} \enskip 
    \chi_S(\alpha) 
    = (-1)^{\sum_{i \in S} \alpha_i}
    = \prod_{i \in S} (-1)^{\alpha_i}
    = \prod_{i \in S} (1 - 2\alpha_i),
\end{equation*}
where the summation is indexed by all the \(2^n\) subsets of \([n] = \{1, \ldots, n\}\).
Each subset \(S \subseteq [n]\) is associated with a \textit{Fourier coefficient} (\textit{weight}) \(\widehat{h}(S) \in \mbb{R}\) and \textit{basis function} \(\chi_S : \{0,1\}^n \to \{-1, + 1\}\).
The definition here is a special case of the \(p\)-biased basis functions, which we describe in~\cref{def:pbiased_basis_functions}.
Expressing a Boolean function in this form makes all the \(k = 0, 1, \ldots, n\) degree interactions between input variables into a linear combination, where the degree of \(\widehat{h}(S) \chi_S (\alpha)\) is the size of \(S\).

These \(\chi_S\) are also known as \textit{parity functions} because they count whether there are an even (\(+1\)) or odd (\(-1\)) number of \(\alpha_i = 1\) for \(i \in S\).
Crucially, they form an orthonormal basis on \(\{0,1\}^n\) via:
\begin{equation*}
    \angles{\chi_S, \chi_T}
    = \expval{\alpha \sim \msf{Bern}(1/2)^n} \bracks*{\chi_S (\alpha) \chi_T (\alpha)}
    = \frac{1}{2^n} \sum_{\alpha \in \{0,1\}^n} \chi_S (\alpha) \chi_T (\alpha)
    = \begin{dcases}
        1, & \text{if \(S = T\)}, \\
        0, & \text{if \(S \neq T\)}.
    \end{dcases}
\end{equation*}
This orthonormality allows each Boolean function to be uniquely expressed as a linear combination of \(\chi_S\) for \(S \subseteq [n]\).
As an example, the function \(h(\alpha_1, \alpha_2) = \alpha_1 \land \alpha_2\) may be uniquely expressed as:
\begin{equation*}
    h(\alpha_1, \alpha_2) = \frac{1}{4} \chi_\emptyset (\alpha) + \frac{1}{4} \chi_{\{1\}} (\alpha) + \frac{1}{4} \chi_{\{2\}} (\alpha) + \frac{1}{4} \chi_{\{1,2\}} (\alpha),
\end{equation*}
where \(\alpha = (\alpha_1, \alpha_2)\), and let \(\chi_\emptyset (\alpha) = 1\) for all \(\alpha\) by convention.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Basic Results in the Standard Basis}


A common strategy for studying operators like \(M_\lambda\) is to inspect how they act on each basis function.
We now present some results with respect to the standard basis functions \(\chi_S\), i.e., the case where \(p = 1/2\).

\begin{lemma} \label{lem:mus_chi}
For any standard basis function \(\chi_S\) and smoothing parameter \(\lambda \in [0,1]\),
\begin{equation*}
    M_\lambda \chi_S (\alpha)
    = \sum_{T \subseteq S}
    \lambda^{\abs{T}} (1 - \lambda)^{\abs{S - T}}  \chi_T (\alpha).
\end{equation*}
\end{lemma}
\begin{proof}
We first expand the definition of \(\chi_S (\alpha)\) to derive:
\begin{align*}
    M_\lambda \chi_S (\alpha)
    % &= \expval{z \sim \msf{Bern}(1/2)^n} \chi_S (\alpha \odot z) \\
    &= \expval{z} \prod_{i \in S} (-1)^{\alpha_i z_i} \\
    &= \prod_{i \in S} \expval{z} (-1)^{\alpha_i z_i}
        \tag{by independence of \(z_1, \ldots, z_n\)} \\
    &= \prod_{i \in S} \bracks*{(1 - \lambda) + \lambda (-1)^{\alpha_i}},
\end{align*}
% where we used the independence of \(z_1, \ldots, z_n\) to swap the expectation and product.
We then use the distributive property to rewrite the product \(\prod_{i \in S} (\cdots)\) as a summation over \(T \subseteq S\) to get
\begin{align*}
    M_\lambda \chi_S (\alpha)
    &= \sum_{T \subseteq S}
        \parens*{\prod_{j \in S - T} (1 - \lambda)}
        \parens*{\prod_{i \in T} \lambda (-1)^{\alpha_i}} \\
    &= \sum_{T \subseteq S} (1 - \lambda)^{\abs{S - T}} \lambda^{\abs{T}} \chi_T (\alpha),
\end{align*}
where \(T\) acts like an enumeration over the \(2^n\) choices of \(z \in \{0,1\}^n\) and recall that \(\chi_T (\alpha) = \prod_{i \in T} (\alpha)\).
\end{proof}

In other words, \(M_\lambda\) redistributes the Fourier weight at each basis \(\chi_S\) over to the \(2^{\abs{S}}\) subsets \(T \subseteq S\) according to a binomial distribution \(\msf{Bin}(\abs{S}, \lambda)\).
Because this redistribution acts linearly on the input, we can visualize \(M_\lambda\) as a \(\mbb{R}^{2^n \times 2^n}\) upper-triangular matrix whose entries are indexed by \(T,S \subseteq [n]\), such that
\begin{equation*}
    (M_\lambda)_{T, S} = \begin{dcases}
        \lambda^{\abs{T}} (1 - \lambda)^{\abs{S - T}}, &\text{if \(T \subseteq S\)}, \\
        0, &\text{otherwise}
    \end{dcases}
\end{equation*}
Using the earlier example of \(h(\alpha_1, \alpha_2) = \alpha_1 \land \alpha_2\), the Fourier coefficients of \(M_\lambda h\) may be expressed as:
\begin{equation*}
    \begin{bmatrix}
        \widehat{M_\lambda h}(\emptyset) \\
        \widehat{M_\lambda h}(\{1\}) \\
        \widehat{M_\lambda h}(\{2\}) \\
        \widehat{M_\lambda h}(\{1,2\})
    \end{bmatrix}
    = \begin{bmatrix}
        1 & (1 - \lambda) & (1 - \lambda) & (1 - \lambda)^2 \\
        & \lambda & & \lambda (1 - \lambda) \\
        & & \lambda & \lambda (1 - \lambda) \\
        & & & \lambda^2
    \end{bmatrix}
    \begin{bmatrix}
        \widehat{h} (\emptyset) \\
        \widehat{h} (\{1\}) \\
        \widehat{h} (\{2\}) \\
        \widehat{h} (\{1,2\})
    \end{bmatrix}
    =
    \frac{1}{4}
    \begin{bmatrix}
        (2 - \lambda)^2 \\
        \lambda (2 - \lambda) \\
        \lambda (2 - \lambda) \\
        \lambda^2
    \end{bmatrix}
\end{equation*}
where recall that \(\widehat{h}(S) = 1/4\) for all \(S \subseteq \{1,2\}\).
In general, it is helpful to lexicographically sort the rows and columns of \(M_\lambda\) and partition them by degree.
As an example with \(n = 3\), one may write \(M_\lambda \in \mbb{R}^{8 \times 8}\) as:
\begin{equation} \label{eqn:m_matrix_example}
M_\lambda \enskip\cong\quad
\begin{array}{c||c|ccc|ccc|c}
    & \emptyset & \{1\} & \{2\} & \{3\} & \{1,2\} & \{1,3\} & \{2,3\} & \{1,2,3\} \\ \hline \hline
\emptyset & 1 & (1-\lambda) & (1-\lambda) & (1-\lambda) & (1-\lambda)^2 & (1-\lambda)^2 & (1-\lambda)^2 & (1-\lambda)^3 \\ \hline
\{1\}     & & \lambda & & & \lambda(1-\lambda) & \lambda(1-\lambda) & & \lambda(1-\lambda)^2 \\
\{2\}     & & & \lambda & & \lambda(1-\lambda) & & \lambda(1-\lambda) & \lambda(1-\lambda)^2 \\
\{3\}     & & & & \lambda & & \lambda(1-\lambda) & \lambda(1-\lambda) & \lambda(1-\lambda)^2 \\ \hline
\{1,2\}   & & & & & \lambda^2 & & & \lambda^2 (1-\lambda) \\
\{1,3\}   & & & & & & \lambda^2 & & \lambda^2 (1-\lambda) \\
\{2,3\}   & & & & & & & \lambda^2 & \lambda^2 (1-\lambda) \\ \hline
\{1,2,3\} & & & & & & & & \lambda^3 \\
\end{array}
\end{equation}

This visualization will help us reason about later proofs.
Because the columns of \(M_\lambda\) sum to \(1\), we have
\begin{equation*}
    \sum_{T \subseteq [n]} \widehat{M_\lambda h}(T) = \sum_{S \subseteq [n]} \widehat{h}(S),
    \quad \text{for any function \(h: \{0,1\}^n \to \mbb{R}\)}.
\end{equation*}
Moreover, \(M_\lambda h\) is a downshift of \(h\) in the sense that: for each \(T \subseteq [n]\), the Fourier coefficient \(\widehat{M_\lambda h}(T)\) depends only on those of \(\widehat{h}(S)\) for \(S \supseteq T\).
This relation is given as follows.


\begin{lemma} \label{lem:mus_h}
For any function \(h: \{0,1\}^n \to \mbb{R}\) and smoothing parameter \(\lambda \in [0,1]\),
\begin{equation*}
    M_\lambda h(\alpha)
    = \sum_{T \subseteq [n]} \widehat{M_\lambda h}(T) \chi_T (\alpha),
    \quad \text{where} \enskip
    \widehat{M_\lambda h}(T)
    = \lambda^{\abs{T}} \sum_{S \supseteq T} (1 - \lambda)^{\abs{S - T}} \widehat{h}(S).
\end{equation*}
\end{lemma}
\begin{proof}
This follows by analyzing the \(T\)-th row of \(M_\lambda\) as in~\cref{eqn:m_matrix_example}.
More specifically, we have:
\begin{align*}
    M_\lambda h(\alpha)
    &= \sum_{S \subseteq [n]} \widehat{h}(S) M_\lambda \chi_S (\alpha) \\
    &= \sum_{S \subseteq [n]} \widehat{h}(S) \sum_{T \subseteq S} \lambda^{\abs{T}} (1 - \lambda)^{\abs{S - T}}  \chi_T (\alpha)
    \tag{\cref{lem:mus_chi}}\\
    &= \sum_{T \subseteq [n]} \chi_T (\alpha) 
    \underbrace{\sum_{S \supseteq T} \lambda ^{\abs{T}} (1 - \lambda)^{\abs{S - T}} \widehat{h}(S)}_{\widehat{M_\lambda h}(T)},
\end{align*}
where the final step follows by noting that each \(\widehat{M_\lambda h}(T)\) depends only on \(\widehat{h}(S)\) for \(S \supseteq T\).
\end{proof}

This expression for \(\widehat{M_\lambda h}(T)\) is useful because it allows us to state a non-trivial contraction result on the spectral mass, i.e., the \(L^1\) norm.
In particular, we give a fine-grained bound on how much mass \(M_\lambda h\) retains for \(\geq k\)-degree terms.

\begin{theorem}[Tail Mass Contraction]
\label{thm:mus_mass_contraction}
For any function \(h: \{0,1\}^n \to \mbb{R}\), smoothing parameter \(\lambda \in [0,1]\), and \(0 \leq k \leq n\),
\begin{equation*}
    \sum_{T: \abs{T} \geq k} \abs{\widehat{M_\lambda h}(T)}
    \leq C(k, n, \lambda)
        \sum_{S: \abs{S} \geq k} \abs{\widehat{h}(S)},
\end{equation*}
where \(C(k, n, \lambda) \leq 1\) is the tail cumulative of \(\msf{Bin}(n, \lambda)\), i.e.,
\(C(k, n, \lambda) = \prob{}[X \geq k]\) for any \(X \sim \msf{Bin}(n, \lambda)\).
\end{theorem}
\begin{proof}
We first apply~\cref{lem:mus_h} to expand each \(\widehat{M_\lambda h}(T)\) and derive
\begin{align*}
    \sum_{T : \abs{T} \geq k} \abs{\widehat{M_\lambda h}(T)}
    &\leq \sum_{T : \abs{T} \geq k} \sum_{S \supseteq T} \lambda^{\abs{T}} (1 - \lambda)^{\abs{S - T}} \abs{\widehat{h}(S)} \\
    &= \sum_{S : \abs{S} \geq k} \abs{\widehat{h}(S)} \underbrace{\sum_{j = k}^{\abs{S}} \binom{\abs{S}}{j} \lambda^{j} (1 - \lambda)^{\abs{S} - j}}_{C(k, \abs{S}, \lambda)}
\end{align*}
where we re-indexed the summations to track the contribution of each \(\abs{\widehat{h}(S)}\) for \(\abs{S} \geq k\).
As a visual aid, we refer to~\cref{eqn:m_matrix_example}.
Finally, applying \(C(k, \abs{S}, \lambda) \leq C(k, n, \lambda)\) yields the stated contraction factor.
\end{proof}


\subsection{Analysis in the Biased Basis}

While analysis on the standard Fourier basis reveals interesting properties about \(M_\lambda\), it suggests that this may not be the natural choice of basis in which to analyze random masking.
Principally, this is because each \(M_\lambda \chi_S\) is expressed as a linear combination of \(\chi_T\) where \(T \subseteq S\).
By ``natural'', we instead aim to express the image of \(M_\lambda\) as a single term.
One partial attempt is an extension of the standard basis, known as the \(p\)-biased basis, which is defined as follows.


\begin{definition}[\(p\)-Biased Basis]
\label{def:pbiased_basis_functions}
For any subset \(S \subseteq [n]\), define its corresponding \(p\)-biased function basis as:
\begin{equation*}
    \chi_S ^p (\alpha) = \prod_{i \in S} \frac{p - \alpha_i}{\sqrt{p - p^2}}.
\end{equation*}
\end{definition}

Observe that when \(p = 1/2\), this is the standard basis discussed earlier.
We first rederive a basic fact that the \(p\)-biased basis functions are orthonormal.

\begin{proposition}[Orthonormality of \(p\)-Biased Basis] \label{prop:chi_S_p_orthonormal}
For any \(p\)-biased basis functions \(\chi_S ^p\) and \(\chi_T ^p\),
\begin{equation*}
    \expval{\alpha \sim \Bern(p)^n} \bracks*{\chi_S ^p (\alpha) \chi_T ^p (\alpha)} = \begin{dcases}
        1, &\text{if \(S = T\)}, \\
        0, &\text{if \(S \neq T\)}.
    \end{dcases}
\end{equation*}
\end{proposition}
\begin{proof}
For any coordinate \(i \in [n]\), note the following identities:
\begin{equation*} % \label{eqn:chi_S_p_orthonormal_1}
    \expval{\alpha \sim \Bern(p)} \bracks*{\frac{p - \alpha_i}{\sqrt{p - p^2}}}
    = 0,
    \quad \expval{\alpha \sim \Bern(p)} \bracks*{\parens*{\frac{p - \alpha_i}{\sqrt{p - p^2}}}^2} = 1.
\end{equation*}
The inner product is then:
\begin{align*}
    \expval{\alpha \sim \Bern(p)^n} \bracks{\chi_S ^p (\alpha) \chi_T ^p (\alpha)}
    &= \expval{\alpha}
    \bracks*{\prod_{i \in S} \frac{p - \alpha_i}{\sqrt{p - p^2}}
    \prod_{j \in T} \frac{p - \alpha_j}{\sqrt{p - p^2}}} \\
    &= \underbrace{\prod_{i \in S \cap T} \expval{\alpha} \bracks*{\parens*{\frac{p - \alpha_i}{\sqrt{p - p^2}}}^2}}_{\text{\(= 1\), for any \(S\) and \(T\)}}
    \underbrace{
    \prod_{j \in S \triangle T} \expval{\alpha} \bracks*{\frac{p - \alpha_j}{\sqrt{p - p^2}}}}_{\text{\(= 0\), if \(S \triangle T \neq \emptyset\)}}
\end{align*}
where we have used the coordinate-wise independence of \(\alpha_1, \ldots, \alpha_n\) to swap the expectation and products.
\end{proof}

On this basis, smoothing with an appropriate choice of \(\lambda\) induces a change-of-basis effect.

\begin{lemma}[Change-of-Basis] \label{lem:M_basis_change}
For any \(p\)-biased basis function \(\chi_S ^p\) and smoothing parameter \(\lambda \in [p, 1]\),
\begin{equation*}
    M_\lambda \chi_S ^p (\alpha)
        = \parens*{\frac{\lambda - p}{1 - p}}^{\abs{S}/2} \chi_S ^{p/\lambda} (\alpha).
\end{equation*}
\end{lemma}
\begin{proof}
Expanding the definition of \(M_\lambda\), we first derive:
\begin{align*}
    M_\lambda \chi_S ^p (\alpha)
    &= \expval{z \sim \Bern(\lambda)^n} \bracks*{\prod_{i \in S} \frac{p - \alpha_i z_i}{\sqrt{p - p^2}}} \\
    &= \prod_{i \in S} \expval{z} \bracks*{\frac{p - \alpha_i z_i}{\sqrt{p - p^2}}} 
        \tag{by independence of \(z_1, \ldots, z_n\)} \\
    &= \prod_{i \in S} \frac{p - \lambda \alpha_i}{\sqrt{p - p^2}},
\end{align*}
% where we swapped the expectation and products using the coordinate-wise independence of \(z_1, \ldots, z_n\).
We then rewrite the above in terms of a \((p/\lambda)\)-biased basis function as follows:
\begin{align*}
    M_\lambda \chi_S ^p (\alpha)
    &= \prod_{i \in S} \lambda \frac{(p/\lambda) - \alpha_i}{\sqrt{p - p^2}} \\
    &= \prod_{i \in S} \lambda \frac{\sqrt{(p/\lambda) - (p/\lambda)^2}}{\sqrt{p - p^2}} \frac{(p/\lambda) - \alpha_i}{\sqrt{(p/\lambda) - (p/\lambda)^2}} \tag{\(\lambda \geq p\)} \\
    &= \prod_{i \in S} \sqrt{\frac{\lambda - p}{1 - p}} \frac{(p/\lambda) - \alpha_i}{\sqrt{(p/\lambda) - (p/\lambda)^2}} \\
    &= \parens*{\frac{\lambda - p}{\sqrt{p - p^2}}}^{\abs{S}/2} \underbrace{\prod_{i \in S} \frac{(p/\lambda) - \alpha_i}{\sqrt{(p/\lambda) - (p/\lambda)^2}}}_{\chi_S ^{p/\lambda} (\alpha)}
\end{align*}
\end{proof}


This change-of-basis makes the variance analysis much more transparent.


\begin{theorem}[Variance Reduction]
For any function \(h: \{0,1\}^n \to \mbb{R}\) and smoothing parameter \(\lambda \in [p, 1]\),
\begin{equation*}
    \variance{\alpha \sim \Bern(p/\lambda)^n} \bracks{M_\lambda h (\alpha)}
    \leq \parens*{\frac{\lambda - p}{1 - p}} \variance{\alpha \sim \Bern(p)^n} \bracks{h(\alpha)}.
\end{equation*}
\end{theorem}
\begin{proof}
We use the previous results to compute:
\begin{align*}
    \variance{\alpha \sim \Bern(p/\lambda)^n} \bracks{M_\lambda h (\alpha)}
    &= \variance{\alpha \sim \Bern(p/\lambda)^n} \bracks*{M_\lambda \sum_{S \subseteq [n]} \widehat{h}(S) \chi_S ^p (\alpha)}
        \tag{by unique \(p\)-biased representation of \(h\)} \\
    &= \variance{\alpha \sim \Bern(p/\lambda)^n} \bracks*{
        \sum_{S \subseteq [n]}
        \parens*{\frac{\lambda - p}{1 - p}}^{\abs{S}/2} \widehat{h}(S) \chi_S ^{p/\lambda} (\alpha)
    } \tag{by linearity and \cref{lem:M_basis_change}} \\
    &= \sum_{S \neq \emptyset} \parens*{\frac{\lambda - p}{1 - p}}^{\abs{S}} \widehat{h}(S)^2
        \tag{Parseval's theorem by orthonormality of \(\chi_S ^{p/\lambda}\)} \\
    &\leq \parens*{\frac{\lambda - p}{1 - p}} \sum_{S \neq \emptyset} \widehat{h}(S)^2 \tag{\(0 \leq \frac{\lambda - p}{1 - p} \leq 1\) because \(p \leq \lambda \leq 1\)} \\
    &= \parens*{\frac{\lambda - p}{1 - p}} \variance{\alpha \sim \Bern(p)^n} [h(\alpha)]
        \tag{Parseval's by orthonormality of \(\chi_S ^p\)}
\end{align*}
\end{proof}


==> old/soft_stability_vs_method.tex <==
\begin{figure}[t]
\centering



\begin{minipage}{0.24\linewidth}
    \centering
    \includegraphics[width=1.0\linewidth]{images/soft_vs_method_vit_imagenet_2_per_class.pdf}
\end{minipage} \hfill
\begin{minipage}{0.24\linewidth}
    \centering
    \includegraphics[width=1.0\linewidth]{images/soft_vs_method_resnet50_imagenet_2_per_class.pdf}
\end{minipage} \hfill
\begin{minipage}{0.24\linewidth}
    \centering
    \includegraphics[width=1.0\linewidth]{images/soft_vs_method_resnet18_imagenet_2_per_class.pdf}
\end{minipage} \hfill
\begin{minipage}{0.24\linewidth}
    \centering
    \includegraphics[width=1.0\linewidth]{images/soft_vs_method_roberta_tweeteval_all.pdf}
\end{minipage}


\caption{
\textbf{Soft stability rate of different explanation methods}.
For ViT, ResNet50, and ResNet18, we used 2000 samples from ImageNet.
For RoBERTa, we used TweetEval.
We used bootstrapping with 1000 iterations to compute a confidence interval of 95\%, shaded.
}
\label{fig:soft_stability_vs_method}
\end{figure}

==> old/stability_vs_smoothing_quantiles.tex <==
\begin{figure*}[t]
\centering

\begin{minipage}{0.19\textwidth}
    \centering
    \includegraphics[width=\linewidth]{images/stability_vs_smoothing_vit_quantiles_1.0.pdf}
\end{minipage}
\hfill
\begin{minipage}{0.19\textwidth}
    \centering
    \includegraphics[width=\linewidth]{images/stability_vs_smoothing_vit_quantiles_0.8.pdf}
\end{minipage}
\hfill
\begin{minipage}{0.19\textwidth}
    \centering
    \includegraphics[width=\linewidth]{images/stability_vs_smoothing_vit_quantiles_0.6.pdf}
\end{minipage}
\hfill
\begin{minipage}{0.19\textwidth}
    \centering
    \includegraphics[width=\linewidth]{images/stability_vs_smoothing_vit_quantiles_0.4.pdf}
\end{minipage}
\hfill
\begin{minipage}{0.19\textwidth}
    \centering
    \includegraphics[width=\linewidth]{images/stability_vs_smoothing_vit_quantiles_0.2.pdf}
\end{minipage}

%%%%%%%%%%%%%%%%%%%%

\begin{minipage}{0.19\textwidth}
    \centering
    \includegraphics[width=\linewidth]{images/stability_vs_smoothing_resnet50_quantiles_1.0.pdf}
\end{minipage}
\hfill
\begin{minipage}{0.19\textwidth}
    \centering
    \includegraphics[width=\linewidth]{images/stability_vs_smoothing_resnet50_quantiles_0.8.pdf}
\end{minipage}
\hfill
\begin{minipage}{0.19\textwidth}
    \centering
    \includegraphics[width=\linewidth]{images/stability_vs_smoothing_resnet50_quantiles_0.6.pdf}
\end{minipage}
\hfill
\begin{minipage}{0.19\textwidth}
    \centering
    \includegraphics[width=\linewidth]{images/stability_vs_smoothing_resnet50_quantiles_0.4.pdf}
\end{minipage}
\hfill
\begin{minipage}{0.19\textwidth}
    \centering
    \includegraphics[width=\linewidth]{images/stability_vs_smoothing_resnet50_quantiles_0.2.pdf}
\end{minipage}


%%%%%%%%%%%%%%%%%%%%

\begin{minipage}{0.19\textwidth}
    \centering
    \includegraphics[width=\linewidth]{images/stability_vs_smoothing_resnet18_quantiles_1.0.pdf}
\end{minipage}
\hfill
\begin{minipage}{0.19\textwidth}
    \centering
    \includegraphics[width=\linewidth]{images/stability_vs_smoothing_resnet18_quantiles_0.8.pdf}
\end{minipage}
\hfill
\begin{minipage}{0.19\textwidth}
    \centering
    \includegraphics[width=\linewidth]{images/stability_vs_smoothing_resnet18_quantiles_0.6.pdf}
\end{minipage}
\hfill
\begin{minipage}{0.19\textwidth}
    \centering
    \includegraphics[width=\linewidth]{images/stability_vs_smoothing_resnet18_quantiles_0.4.pdf}
\end{minipage}
\hfill
\begin{minipage}{0.19\textwidth}
    \centering
    \includegraphics[width=\linewidth]{images/stability_vs_smoothing_resnet18_quantiles_0.2.pdf}
\end{minipage}


%%%%%%%%%%%%%%%%%%%%

\begin{minipage}{0.19\textwidth}
    \centering
    \includegraphics[width=\linewidth]{images/stability_vs_smoothing_roberta_quantiles_1.0.pdf}
\end{minipage}
\hfill
\begin{minipage}{0.19\textwidth}
    \centering
    \includegraphics[width=\linewidth]{images/stability_vs_smoothing_roberta_quantiles_0.8.pdf}
\end{minipage}
\hfill
\begin{minipage}{0.19\textwidth}
    \centering
    \includegraphics[width=\linewidth]{images/stability_vs_smoothing_roberta_quantiles_0.6.pdf}
\end{minipage}
\hfill
\begin{minipage}{0.19\textwidth}
    \centering
    \includegraphics[width=\linewidth]{images/stability_vs_smoothing_roberta_quantiles_0.4.pdf}
\end{minipage}
\hfill
\begin{minipage}{0.19\textwidth}
    \centering
    \includegraphics[width=\linewidth]{images/stability_vs_smoothing_roberta_quantiles_0.2.pdf}
\end{minipage}



% \begin{minipage}{0.24\textwidth}
%     \centering
%     \includegraphics[width=\linewidth]{images/resnet_stability_vs_lambda_alpha0.10.pdf}
% \end{minipage}
% \hfill
% \begin{minipage}{0.24\textwidth}
%     \centering
%     \includegraphics[width=\linewidth]{images/resnet_stability_vs_lambda_alpha0.15.pdf}
% \end{minipage}
% \hfill
% \begin{minipage}{0.24\textwidth}
%     \centering
%     \includegraphics[width=\linewidth]{images/resnet_stability_vs_lambda_alpha0.20.pdf}
% \end{minipage}
% \hfill
% \begin{minipage}{0.24\textwidth}
%     \centering
%     \includegraphics[width=\linewidth]{images/resnet_stability_vs_lambda_alpha0.20.pdf}
% \end{minipage}

% %%%%%%%%%%%%%%%%%%%%

% \begin{minipage}{0.24\textwidth}
%     \centering
%     \includegraphics[width=\linewidth]{images/roberta_stability_vs_lambda_alpha0.10.pdf}
% \end{minipage}
% \hfill
% \begin{minipage}{0.24\textwidth}
%     \centering
%     \includegraphics[width=\linewidth]{images/roberta_stability_vs_lambda_alpha0.15.pdf}
% \end{minipage}
% \hfill
% \begin{minipage}{0.24\textwidth}
%     \centering
%     \includegraphics[width=\linewidth]{images/roberta_stability_vs_lambda_alpha0.20.pdf}
% \end{minipage}
% \hfill
% \begin{minipage}{0.24\textwidth}
%     \centering
%     \includegraphics[width=\linewidth]{images/roberta_stability_vs_lambda_alpha0.20.pdf}
% \end{minipage}

\caption{
\textbf{Smoothing can improve stability, but there is noise.}
Principally, this is because different input samples have different stability rates with respect to our random selection of 25\% of the features as the attribution.
We plot the median and inter-quartile range (25\%-75\%) of the stability rate across different perturbation radii for various values of \(\lambda\).
We used 200 samples from ImageNet and 200 samples from TweetEval that had at least 40 tokens.
}
\label{fig:stability_vs_smoothing_quantiles}
\end{figure*}

==> sections/icml_statements.tex <==

\section*{Impact Statement}

This paper presents work whose goal is to advance the field of Machine Learning by making machine learning models more interpretable and trustworthy to human practitioners. There are many potential societal consequences of our work, none which we feel must be specifically highlighted here.
